If there is no underfitting, there is no Cold Posterior Effect

The cold posterior effect (CPE) (Wenzel et al., 2020) in Bayesian deep learning shows that, for posteriors with a temperature $T<1$, the resulting posterior predictive could have better performances than the Bayesian posterior ($T=1$). As the Bayesian posterior is known to be optimal under perfect model specification, many recent works have studied the presence of CPE as a model misspecification problem, arising from the prior and/or from the likelihood function. In this work, we provide a more nuanced understanding of the CPE as we show that misspecification leads to CPE only when the resulting Bayesian posterior underfits. In fact, we theoretically show that if there is no underfitting, there is no CPE.

==> contents/App-variational-decomposition.tex <==
We take a prior from the family of factorized distribution, i.e., $p(\bmtheta)=\prod_{i=1}^M p_i(\theta_i)$. We consider the variational posterior $q(\bmtheta)$ that approximate the posterior $p_\ell^\lambda(\bmtheta|D)$ and can be factorized by $\prod_{i=1}^M q_i(\theta_i)$. It is then known that 

\[ 
q_i(\theta_i) = \frac{p_i(\theta_i)e^{\lambda h(D,\theta_i)}}{\int p_i(\theta_i)e^{\lambda h(D,\theta_i) }d\theta_i} \propto e^{\lambda h(D,\theta_i) + \ln p_i(\theta_i)},
\]
where
\[h(D,\theta_i) = \mathbb{E}_{j\neq i}[\ln p(D|\bmtheta)]=\int \prod_{j\neq i} q_j(\theta_j) \ln p(D|\bmtheta) d\bmtheta_{-i}. \]

\paragraph{Gradient of the Gibbs loss} Let's now derive the gradient of the Gibbs loss with such a factorized posterior. For any function $f$, 
\[
\nabla_\lambda \E_{q}[f(\bmtheta)]=\nabla_\lambda \lr{\int \prod_{i=1}^M q_i(\theta_i) f(\bmtheta)d\bmtheta} =\int  \nabla_\lambda \lr{\prod_{i=1}^M q_i(\theta_i) }f(\bmtheta)d\bmtheta = \int \sum_{i=1}^M \nabla_\lambda q_i(\theta_i)\prod_{j\neq i} q_j(\theta_j) f(\bmtheta)d\bmtheta.
\]
Since for any $i\in[M]$, the gradient of the posterior   
$\nabla_\lambda q_i(\theta_i)=h(D,\theta_i)q_i(\theta_i)-q_i(\theta_i)\E_{q_i}[h(D,\theta_i)]$, the above expression
\begin{align*}
    \int \sum_{i=1}^M \nabla_\lambda q_i(\theta_i)\prod_{j\neq i} q_j(\theta_j) f(\bmtheta)d\bmtheta &= \int \sum_{i=1}^M\lr{h(D,\theta_i)q_i(\theta_i)-q_i(\theta_i)\E_{q_i}[h(D,\theta_i)]}\prod_{j\neq i} q_j(\theta_j) f(\bmtheta)d\bmtheta\\
    &= \int \sum_{i=1}^M\lr{h(D,\theta_i)-\E_{q_i}[h(D,\theta_i)]}\prod_{j=1}^M q_j(\theta_j) f(\bmtheta)d\bmtheta\\
    &=  \sum_{i=1}^M\int\lr{h(D,\theta_i)-\E_{q_i}[h(D,\theta_i)]}\prod_{j=1}^M q_j(\theta_j) f(\bmtheta)d\bmtheta\\
    &= \sum_{i=1}^M \lr{\E_q [h(D,\theta_i)f(\bmtheta)] - \E_{q_i}[h(D,\theta_i)]\E_q[f(\bmtheta)] }\\
    &=\sum_{i=1}^M \lr{\E_q [h(D,\theta_i)f(\bmtheta)] - \E_{q}[h(D,\theta_i)]\E_q[f(\bmtheta)] }\\
    &=\sum_{i=1}^M \mathbb{COV}_q\lr{h(D,\theta_i),f(\bmtheta)}.
\end{align*}
Hence, we conclude that for the factorized variational posterior 
$q(\bmtheta)$, the gradient of the Gibbs loss $\nabla_\lambda\E_q[f(\bmtheta)]=\sum_{i=1}^M \mathbb{COV}_q\lr{h(D,\theta_i),f(\bmtheta)}$, where $h(D,\theta_i) = \mathbb{E}_{j\neq i}[\ln p(D|\bmtheta)]$. 

\paragraph{Gradient of the Bayes loss} By definition,
\begin{equation*}
    \nabla_\lambda B(q) = \nabla_\lambda \E_\nu\lrs{-\ln\E_q[p(\bmy|\bmx,\bmtheta)] } = -\E_\nu\lrs{\nabla_\lambda \ln\E_q[p(\bmy|\bmx,\bmtheta) ] },
\end{equation*}
where
\begin{equation*}
    \nabla_\lambda \ln\E_q[p(\bmy|\bmx,\bmtheta) ] = \frac{\nabla_\lambda \E_q[p(\bmy|\bmx,\bmtheta)]}{\E_q[p(\bmy|\bmx,\bmtheta)]} = \frac{\sum_{i=1}^M \mathbb{COV}_q\lr{h(D,\theta_i),p(\bmy|\bmx,\bmtheta)} }{\E_q[p(\bmy|\bmx,\bmtheta)]}
\end{equation*}
due to the conclusion above for the gradient of the Gibbs loss with $f(\bmtheta)=p(\bmy|\bmx,\bmtheta)$.

\iffalse
\[p^\lambda_M(\bmtheta|D) = p^\lambda_1(\theta_1|D)\cdot\ldots\cdot p^\lambda_K(\theta_K|D) \]
\[p(\bmtheta) = \prod_i p(\theta_i)\]

\[ p^\lambda_i(\theta_i|D) = \frac{p(\theta_i)e^{\lambda g(D,\theta_i)}}{\int p(\theta_i)e^{\lambda g(D,\theta_i) d\theta_i}} \]

\[g(D,\theta_i) = \mathbb{E}_{j\neq i}[\ln p(D|\bmtheta)]= \mathbb{E}_{j\neq i}[\ln p(D|\theta_1,\ldots,\theta_M)] =\int \prod_{j\neq i} p^\lambda_j(\theta_j|D) \ln p(D|\theta_1,\ldots,\theta_M) d\bmtheta \]


\[\nabla_\lambda \E_{p^\lambda_M}[f(\bmtheta)] =  \int  \nabla_\lambda  \prod_{i} p^\lambda_i(\theta_i|D) f(\bmtheta) d\bmtheta = Cov_{p^\lambda_M}(\sum_i g(D,\theta_i),f(\bmtheta))\]
\fi

\newpage



\begin{eqnarray}
q^\lambda(\bmtheta) &= \argmin_{\rho_1,\ldots,\rho_M} \E_\rho[-\ln p(D|\bmtheta)] + \frac{1}{\lambda}\sum_j KL(\rho_j(\theta_j),p_j(\theta_j))\\
\end{eqnarray}


\[ q(\lambda) = \argmin_q g(q,\lambda)\]

\[ \nabla_\lambda g(q(\lambda),\lambda) = \nabla_q g(q,\lambda)_{|q=q(\lambda)}\nabla_\lambda g(\lambda) + \nabla_\lambda g(q,\lambda)_{|q=q(\lambda)} = \nabla_\lambda g(q,\lambda)_{|q=q(\lambda)} \]

==> hl_short.tex <==
\usepackage{xspace}
\usepackage{graphics,graphicx,epsfig}
\usepackage{url}

\newcommand{\nc}{\newcommand}

%      HELGE's EGNE "NEWCOMMANDS"



%%      THEOREMER OG SLIKT%
%
\newtheorem{hl_example}{Example}
\newtheorem{hl_algorithm}{Algorithm}
\newtheorem{hl_theorem}{Theorem}
\newtheorem{hl_proposition}{Proposition}
\newtheorem{hl_lemma}{Lemma}
\newtheorem{hl_corollary}{Corollary}
\newtheorem{hl_definition}{Definition}
\newtheorem{hl_conjecture}{Conjecture}
\newenvironment{hl_nonumberenv}[1]{{\bf #1}\begin{it}}{\end{it}}
\newtheorem{hl_proof}{Proof}



%      KOMMENTARMARKERING

\nc{\vekk}[1]{}   %         \vekk{Brukes for � markere vekk tekst}
%\nc{\comment}[1]{\mbox{}\marginpar{\raggedright\hspace{0pt}#1}}%
\nc{\hl}[1]{\comment{{\bf HL:} #1}} %
\nc{\tdn}[1]{\comment{{\bf TDN:} #1}} %



%      BEGIN/END

\nc{\bex}{\begin{example}} \nc{\eex}{\end{example}}

%\nc{\bth}{\begin{theorem}}
%\nc{\eth}{\end{theorem}}

\nc{\ble}{\begin{lemma}}
\nc{\ele}{\end{lemma}}

\nc{\bco}{\begin{conjecture}}
\nc{\eco}{\end{conjecture}}

\nc{\beq}{\begin{equation}}
\nc{\eeq}{\end{equation}}

\nc{\beqa}{\begin{eqnarray}}
\nc{\eeqa}{\end{eqnarray}}

\nc{\beqas}{\begin{eqnarray*}}%
\nc{\eeqas}{\end{eqnarray*}}

\nc{\bsp}{\[\begin{array}{rcl}}
\nc{\esp}{\end{array}\]}

\nc{\btab}[1]{\begin{tabular}{#1}}
\nc{\etab}{\end{tabular}}

\nc{\bfi}{\begin{figure}[htpb]}
\nc{\efi}{\end{figure}}

\nc{\ben}{\begin{enumerate}}
\nc{\een}{\end{enumerate}}

\nc{\bit}{\begin{itemize}}
\nc{\eit}{\end{itemize}}

\nc{\bde}{\begin{description}}
\nc{\ede}{\end{description}}


%      PRODUKT, BINOMISKE TING OG SUMMER

\nc{\pin}{\prod_{i=1}^n} \nc{\pjm}{\prod_{j=1}^m}
\nc{\pkm}{\prod_{k=1}^m} \nc{\pjM}{\prod_{j=1}^M}
\nc{\suin}{\sum_{i=1}^n} \nc{\sujm}{\sum_{j=1}^m}
\nc{\sukm}{\sum_{k=1}^m} \nc{\sujM}{\sum_{j=1}^M} \nc{\bimr}{\left
(_r^m \right)} \nc{\birs}{\left (_s^r \right)}
\nc{\bin}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%      CAL-TING
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\nc{\cal}{\mathcal}

\nc{\calDelta}{\mbox{$\cal{\Delta}$}}

% \nc{\calA}{\mbox{${\cal A}$}} \nc{\calB}{\mbox{$\cal{B}$}}
% \nc{\calC}{\mbox{$\cal{C}$}} \nc{\calD}{\mbox{$\cal{D}$}}
% \nc{\calE}{\mbox{$\cal{E}$}} \nc{\calF}{\mbox{$\cal{F}$}}
% \nc{\calG}{\mbox{$\cal{G}$}} \nc{\calH}{\mbox{$\cal{H}$}}
% \nc{\calI}{\mbox{$\cal{I}$}} \nc{\calJ}{\mbox{$\cal{J}$}}
% \nc{\calK}{\mbox{$\cal{K}$}} \nc{\calL}{\mbox{$\cal{L}$}}
% \nc{\calM}{\mbox{$\cal{M}$}} \nc{\calN}{\mbox{$\cal{N}$}}
% \nc{\calO}{\mbox{$\cal{O}$}} \nc{\calP}{\mbox{$\cal{P}$}}
% \nc{\calQ}{\mbox{$\cal{Q}$}} \nc{\calR}{\mbox{$\cal{R}$}}
% \nc{\calS}{\mbox{$\cal{S}$}} \nc{\calT}{\mbox{$\cal{T}$}}
% \nc{\calU}{\mbox{$\cal{U}$}} \nc{\calV}{\mbox{$\cal{V}$}}
% \nc{\calW}{\mbox{$\cal{W}$}} \nc{\calX}{\mbox{$\cal{X}$}}
% \nc{\calY}{\mbox{$\cal{Y}$}} \nc{\calZ}{\mbox{$\cal{Z}$}}
% \nc{\calz}{\mbox{$\cal{z}$}}



\nc{\calA}{{\ensuremath{\cal{A}}}} \nc{\calB}{{\ensuremath{\cal{B}}}}
\nc{\calC}{{\ensuremath{\cal{C}}}} \nc{\calD}{{\ensuremath{\cal{D}}}}
\nc{\calE}{{\ensuremath{\cal{E}}}} \nc{\calF}{{\ensuremath{\cal{F}}}}
\nc{\calG}{{\ensuremath{\cal{G}}}} \nc{\calH}{{\ensuremath{\cal{H}}}}
\nc{\calI}{{\ensuremath{\cal{I}}}} \nc{\calJ}{{\ensuremath{\cal{J}}}}
\nc{\calK}{{\ensuremath{\cal{K}}}} \nc{\calL}{{\ensuremath{\cal{L}}}}
\nc{\calM}{{\ensuremath{\cal{M}}}} \nc{\calN}{{\ensuremath{\cal{N}}}}
\nc{\calO}{{\ensuremath{\cal{O}}}} \nc{\calP}{{\ensuremath{\cal{P}}}}
\nc{\calQ}{{\ensuremath{\cal{Q}}}} \nc{\calR}{{\ensuremath{\cal{R}}}}
\nc{\calS}{{\ensuremath{\cal{S}}}} \nc{\calT}{{\ensuremath{\cal{T}}}}
\nc{\calU}{{\ensuremath{\cal{U}}}} \nc{\calV}{{\ensuremath{\cal{V}}}}
\nc{\calW}{{\ensuremath{\cal{W}}}} \nc{\calX}{{\ensuremath{\cal{X}}}}
\nc{\calY}{{\ensuremath{\cal{Y}}}} \nc{\calZ}{{\ensuremath{\cal{Z}}}}
\nc{\calz}{{\ensuremath{\cal{z}}}}



%\nc{\NP}{\mbox{$\calN\calP$}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%      BOLDMATH-TING
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\nc{\bm}{\boldmath}
% \nc{\bm}{\bf}
\nc{\bma}{{\ensuremath{\boldsymbol{a}}}} 
\nc{\bmb}{{\ensuremath{\boldsymbol{b}}}}
\nc{\bmc}{{\ensuremath{\boldsymbol{c}}}} \nc{\bmd}{{\ensuremath{\boldsymbol{d}}}}
\nc{\bme}{{\ensuremath{\boldsymbol{e}}}} \nc{\bmf}{{\ensuremath{\boldsymbol{f}}}}
\nc{\bmg}{{\ensuremath{\boldsymbol{g}}}} \nc{\bmh}{{\ensuremath{\boldsymbol{h}}}}
\nc{\bmi}{{\ensuremath{\boldsymbol{i}}}} \nc{\bmj}{{\ensuremath{\boldsymbol{j}}}}
\nc{\bmk}{{\ensuremath{\boldsymbol{k}}}} \nc{\bml}{{\ensuremath{\boldsymbol{l}}}}
\nc{\bmm}{{\ensuremath{\boldsymbol{m}}}} \nc{\bmn}{{\ensuremath{\boldsymbol{n}}}}
\nc{\bmo}{{\ensuremath{\boldsymbol{o}}}} \nc{\bmp}{{\ensuremath{\boldsymbol{p}}}}
\nc{\bmq}{{\ensuremath{\boldsymbol{q}}}} \nc{\bmr}{{\ensuremath{\boldsymbol{r}}}}
\nc{\bms}{{\ensuremath{\boldsymbol{s}}}} \nc{\bmt}{{\ensuremath{\boldsymbol{t}}}}
\nc{\bmu}{{\ensuremath{\boldsymbol{u}}}} \nc{\bmv}{{\ensuremath{\boldsymbol{v}}}}
\nc{\bmw}{{\ensuremath{\boldsymbol{w}}}} \nc{\bmx}{{\ensuremath{\boldsymbol{x}}}}
\nc{\bmy}{{\ensuremath{\boldsymbol{y}}}} \nc{\bmz}{{\ensuremath{\boldsymbol{z}}}}

% \nc{\bma}{{\mbox{\bm $a$}}} 
% \nc{\bmb}{{\mbox{\bm $b$}}}
% \nc{\bmc}{{\mbox{\bm $c$}}} \nc{\bmd}{{\mbox{\bm $d$}}}
% \nc{\bme}{{\mbox{\bm $e$}}} \nc{\bmf}{{\mbox{\bm $f$}}}
% \nc{\bmg}{{\mbox{\bm $g$}}} \nc{\bmh}{{\mbox{\bm $h$}}}
% \nc{\bmi}{{\mbox{\bm $i$}}} \nc{\bmj}{{\mbox{\bm $j$}}}
% \nc{\bmk}{{\mbox{\bm $k$}}} \nc{\bml}{{\mbox{\bm $l$}}}
% \nc{\bmm}{{\mbox{\bm $m$}}} \nc{\bmn}{{\mbox{\bm $n$}}}
% \nc{\bmo}{{\mbox{\bm $o$}}} \nc{\bmp}{{\mbox{\bm $p$}}}
% \nc{\bmq}{{\mbox{\bm $q$}}} \nc{\bmr}{{\mbox{\bm $r$}}}
% \nc{\bms}{{\mbox{\bm $s$}}} \nc{\bmt}{{\mbox{\bm $t$}}}
% \nc{\bmu}{{\mbox{\bm $u$}}} \nc{\bmv}{{\mbox{\bm $v$}}}
% \nc{\bmw}{{\mbox{\bm $w$}}} \nc{\bmx}{{\mbox{\bm $x$}}}
% \nc{\bmy}{{\mbox{\bm $y$}}} \nc{\bmz}{{\mbox{\bm $z$}}}


\nc{\bmA}{{\ensuremath{\boldsymbol{A}}}} \nc{\bmB}{{\ensuremath{\boldsymbol{B}}}}
\nc{\bmC}{{\ensuremath{\boldsymbol{C}}}} \nc{\bmD}{{\ensuremath{\boldsymbol{D}}}}
\nc{\bmE}{{\ensuremath{\boldsymbol{E}}}} \nc{\bmF}{{\ensuremath{\boldsymbol{F}}}}
\nc{\bmG}{{\ensuremath{\boldsymbol{G}}}} \nc{\bmH}{{\ensuremath{\boldsymbol{H}}}}
\nc{\bmI}{{\ensuremath{\boldsymbol{I}}}} \nc{\bmJ}{{\ensuremath{\boldsymbol{J}}}}
\nc{\bmK}{{\ensuremath{\boldsymbol{K}}}} \nc{\bmL}{{\ensuremath{\boldsymbol{L}}}}
\nc{\bmM}{{\ensuremath{\boldsymbol{M}}}} \nc{\bmN}{{\ensuremath{\boldsymbol{N}}}}
\nc{\bmO}{{\ensuremath{\boldsymbol{O}}}} \nc{\bmP}{{\ensuremath{\boldsymbol{P}}}}
\nc{\bmQ}{{\ensuremath{\boldsymbol{Q}}}} \nc{\bmR}{{\ensuremath{\boldsymbol{R}}}}
\nc{\bmS}{{\ensuremath{\boldsymbol{S}}}} \nc{\bmT}{{\ensuremath{\boldsymbol{T}}}}
\nc{\bmU}{{\ensuremath{\boldsymbol{U}}}} \nc{\bmV}{{\ensuremath{\boldsymbol{V}}}}
\nc{\bmW}{{\ensuremath{\boldsymbol{W}}}} \nc{\bmX}{{\ensuremath{\boldsymbol{X}}}}
\nc{\bmY}{{\ensuremath{\boldsymbol{Y}}}} \nc{\bmZ}{{\ensuremath{\boldsymbol{Z}}}}

% \nc{\bmA}{{\mbox{\bm $A$}}} \nc{\bmB}{{\mbox{\bm $B$}}}
% \nc{\bmC}{{\mbox{\bm $C$}}} \nc{\bmD}{{\mbox{\bm $D$}}}
% \nc{\bmE}{{\mbox{\bm $E$}}} \nc{\bmF}{{\mbox{\bm $F$}}}
% \nc{\bmG}{{\mbox{\bm $G$}}} \nc{\bmH}{{\mbox{\bm $H$}}}
% \nc{\bmI}{{\mbox{\bm $I$}}} \nc{\bmJ}{{\mbox{\bm $J$}}}
% \nc{\bmK}{{\mbox{\bm $K$}}} \nc{\bmL}{{\mbox{\bm $L$}}}
% \nc{\bmM}{{\mbox{\bm $M$}}} \nc{\bmN}{{\mbox{\bm $N$}}}
% \nc{\bmO}{{\mbox{\bm $O$}}} \nc{\bmP}{{\mbox{\bm $P$}}}
% \nc{\bmQ}{{\mbox{\bm $Q$}}} \nc{\bmR}{{\mbox{\bm $R$}}}
% \nc{\bmS}{{\mbox{\bm $S$}}} \nc{\bmT}{{\mbox{\bm $T$}}}
% \nc{\bmU}{{\mbox{\bm $U$}}} \nc{\bmV}{{\mbox{\bm $V$}}}
% \nc{\bmW}{{\mbox{\bm $W$}}} \nc{\bmX}{{\mbox{\bm $X$}}}
% \nc{\bmY}{{\mbox{\bm $Y$}}} \nc{\bmZ}{{\mbox{\bm $Z$}}}




\nc{\bmUpsilon}{{\mbox{\bm $\boldsymbol{\Upsilon}$}}}
\nc{\bmupsilon}{{\mbox{\bm $\boldsymbol{\upsilon}$}}}
\nc{\bmalpha}{{\mbox{\bm $\boldsymbol{\alpha}$}}}
\nc{\bmbeta}{{\mbox{\bm $\boldsymbol{\beta}$}}}
\nc{\bmgamma}{{\mbox{\bm $\boldsymbol{\gamma}$}}}
\nc{\bmGamma}{{\mbox{\bm $\boldsymbol{\Gamma}$}}}
\nc{\bmdelta}{{\mbox{\bm $\boldsymbol{\delta}$}}}
\nc{\bmDelta}{{\mbox{\bm $\boldsymbol{\Delta}$}}}
\nc{\bmeps}{{\mbox{\bm $\boldsymbol{\epsilon}$}}}
\nc{\bmepsilon}{\bmeps}
\nc{\bmphi}{{\mbox{\bm $\boldsymbol{\phi}$}}}
\nc{\bmPhi}{{\mbox{\bm $\$\boldsymbol{\Phi}$}}}
\nc{\bmlambda}{{\mbox{\bm $\boldsymbol{\lambda}$}}}
\nc{\bmLambda}{{\mbox{\bm $\boldsymbol{\Lambda}$}}}
\nc{\bmmu}{{\mbox{\bm $\boldsymbol{\mu}$}}}
\nc{\bmnu}{{\mbox{\bm $\boldsymbol{\nu}$}}}
\nc{\bmpi}{{\mbox{\bm $\boldsymbol{\pi}$}}}
\nc{\bmrho}{{\mbox{\bm$\boldsymbol{\rho}$}}}
\nc{\bmpsi}{{\mbox{\bm $\boldsymbol{\psi}$}}}
\nc{\bmPsi}{{\mbox{\bm $\boldsymbol{\Psi}$}}}
\nc{\bmsigma}{{\mbox{\bm $\boldsymbol{\sigma}$}}}
\nc{\bmSigma}{{\mbox{\bm $\boldsymbol{\Sigma}$}}}
\nc{\bmtheta}{{\ensuremath{\boldsymbol{\theta}}}}
%\nc{\bmTheta}{{\mbox{\bm $\Theta$}}}
\nc{\bmTheta}{{\ensuremath{\boldsymbol{\Theta}}}}
\nc{\bmeta}{{\ensuremath{\boldsymbol{\eta}}}}
\nc{\bmzeta}{{\mbox{\bm $\zeta$}}}
\nc{\bmxi}{{\mbox{\bm $\xi$}}} \nc{\bmXi}{{\mbox{\bm $\Xi$}}}
\nc{\bmnabla}{{\mbox{\bm $\nabla$}}}
\nc{\bmomega}{{\mbox{\bm $\omega$}}}
\nc{\bmOmega}{{\mbox{\bm $\Omega$}}}

\nc{\bmen}{{\bf 1}} \nc{\bmhalf}{{\bf\frac{1}{2}}}
\nc{\bmnull}{{\bf \ensuremath{0}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% General terminology
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nc{\Var}{\mbox{Var}} \nc{\Cov}{\mbox{Cov}}
\nc{\E}{\mbox{$\mathbb{E}$}}
\nc{\KL}[2]{D\left(\,#1\,\norm\,#2\,\right)}
\nc{\convL}{\stackrel{\calL}{\rightarrow}} \nc{\given}{|}
%\nc{\norm}{||}
\nc{\norm}{\|} \nc{\sizeof}[1]{\left|#1\right|}

\nc{\iffp}{\mbox{$\Leftrightarrow$}} \nc{\ien}{\mbox{$i=1\ld n$}}
%\nc{\R}{\mbox{$\mathbb{R}$}}
\nc{\nat}{\mbox{$\mathbb{N}$}} \nc{\infinity}{\infty}
\nc{\ld}{,\ldots,} \nc{\defi}{:=} \nc{\incl}{\subset}
\nc{\upin}[2]{#1^{(#2)}} \nc{\non}{\nonumber}
\nc{\stless}{\stackrel{\mbox{st}}{\leq}}
\gdef\qed{\relax\ifmmode~\hfill\square\else\unskip\nobreak
    ~\hfill$\square$\fi}
\nc{\boxen}{\begin{flushright}$\rule{3mm}{3mm}$\end{flushright}}
\newcommand{\trans}{^{\mbox{\tiny{T}}}}
%\newcommand{\trans}{\top}
\newcommand{\T}{\trans}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Special reliability analysis
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nc{\h}{\mbox{$h(\bmp)$}}
\nc{\hm}{\mbox{$h^m(\bmp)$}}
\nc{\hnei}{\mbox{$h({\bf p})$}}
\nc{\hmnei}{\mbox{$h^m({\bf p})$}}
\nc{\hj}{h_j(\bmp)}
\nc{\hmj}{h_j^m(\bmp)}
\nc{\hjm}{\hmj}
\nc{\ph}{\phi(\bmx)}
\nc{\Ph}{\phi(\bmX)}
%\nc{\p}{\overline P}
\nc{\ip}{\coprod}
\nc{\phd}{\phi^D (\bmx)}
\nc{\Phd}{\phi^D(\bmX)}
\nc{\hd}{h^D (\bmp)}
\nc{\hdm}{\left( h^D (\bmp) \right)^m}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BN related stuff
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \nc{\pa}[1]{{\rm pa}\left(#1\right)}
 \nc{\mb}[1]{{\rm mb}\left(#1\right)}
 \nc{\sspace}[1]{\ensuremath{sp\left(#1\right)}}
% \nc{\sspace}[1]{{\rm sp}\left(#1\right)}
 \nc{\child}[1]{\mbox{${\rm ch}\left(#1\right)$}}
 \nc{\indep}{\mbox{$\perp\!\!\!\perp$}}
 \nc{\nonindep}{\not\!\!\!\indep} \nc{\NB}{Na\"{\i}ve Bayes\xspace}
 \nc{\nB}{na\"{\i}ve Bayes\xspace}
 \nc{\MDL}{\mbox{MDL}\xspace} \nc{\MDLp}{$\mbox{MDL}_p$\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This part here for the HuginToPsTrics stuff by Thomas
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Fbox}[5][0.5cm]{\rput(#2,#3){\rnode{#4}{\psframebox{\parbox[c][#1]{#1}{\centerline{#5}}}}}}
\newcommand{\Fnode}[5][0.5cm]{\cnodeput[doubleline=false](#2,#3){#4}{\makebox[#1]{#5}}}
\newcommand{\FDblnode}[5][0.5cm]{\cnodeput[doubleline=true](#2,#3){#4}{\makebox[#1]{#5}}}
\newcommand{\Fdiam}[5][0.3cm]{\rput(#2,#3){\dianode{#4}{\makebox[#1]{#5}}}}
\newcommand{\Fovalnode}[5][0.5cm]{\rput(#2,#3){\ovalnode{#4}{\makebox[#1]{#5}}}}
\newcommand{\FDblovalnode}[5][0.5cm]{\rput(#2,#3){\ovalnode[doubleline=true]{#4}{\makebox[#1]{#5}}}}
\newcommand{\Frect}[5][0.5cm]{\rput(#2,#3){\rnode{#4}{\psframebox{\makebox[#1]{#5}}}}}
\newcommand{\arc}[3][solid]{\ncline[linestyle=#1]{->}{#2}{#3}}
%\newpsobject{showgrid}{psgrid}{subgriddiv=1,griddots=10,gridlabels=6pt}
%\psset{unit=0.5cm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% pstexfig: Latex-type figures from xfig.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\pstexfig}[2] {
\begin{nopagebreak}
  \begin{figure}[htpb]
    \begin{center}
      \input{./FIGS/#1.pstex_t}
        \caption{#2}
      \label{fig:#1}
    \end{center}
  \end{figure}
\end{nopagebreak}
}

\newcommand{\pstexFig}[2] {
\begin{nopagebreak}
  \begin{figure*}[htbp]
    \begin{center}
      \input{./FIGS/#1.pstex_t}
        \caption{#2}
      \label{fig:#1}
    \end{center}
  \end{figure*}
\end{nopagebreak}
}

\newcommand{\pstexfigSlide}[1] {
\begin{nopagebreak}
    \begin{center}
        \input{./#1.pstex_t}
    \end{center}
\end{nopagebreak}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% epsfigur: Get an eps-fig from file
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\epsfigur}[3] {
\begin{nopagebreak}
  \begin{figure}[htpb]
    \begin{center}
      \epsfig{file =./FIGS/#1.eps,width=#3mm}
        \caption{#2}
      \label{fig:#1}
    \end{center}
  \end{figure}
\end{nopagebreak}
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% psfigur: Get an ps-fig from file
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\psfigur}[3] {
\begin{nopagebreak}
  \begin{figure}[htpb]
    \begin{center}
      \psfig{file =./FIGS/#1.ps,width=#3mm,angle=-90}
       \caption{#2}
      \label{fig:#1}
    \end{center}
  \end{figure}
\end{nopagebreak}
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Rpsfigur: Get an ps-fig from file
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Rpsfigur}[3] {
\begin{nopagebreak}
  \begin{figure}[htpb]
    \begin{center}
      \psfig{file =./FIGS/#1.ps,width=#3mm}
       \caption{#2}
      \label{fig:#1}
    \end{center}
  \end{figure}
\end{nopagebreak}
}



\nc{\figref}[1]{\figurename~\ref{fig:#1}\xspace}
\nc{\tabref}[1]{Table~\ref{tab:#1}\xspace}
\nc{\equref}[1]{Equation~(\ref{equ:#1})\xspace}
\nc{\secref}[1]{Section~\ref{sec:#1}\xspace}
\nc{\algoref}[1]{Algorithm~\ref{algo:#1}\xspace}
\nc{\stepref}[1]{Step~\ref{step:#1}\xspace}

\nc{\includebib}{\bibliography{defs,%
                               hl,%
                               master,%
                               dynamic,%
                               reliability,%
                               troubleshoot,%
                               class,%
                               learning,%
                               luigi,%
			      footy,%
                               antonio,%
%                               mte,%
                               global%
}}


==> meta-proof-gradient.tex <==
We will derive a meta-analysis and later apply it to posteriors from different tempering methods.

\paragraph{Gradient of the Gibbs loss}
We first show a general result of the gradient of the Gibbs loss, $\nabla\E_\rho[f(\bmtheta)]$, for any function $f(\bmtheta)$ that is independent of $\lambda$, $\gamma$, and $\tau$, and posterior with the form $\rho(\bmtheta|D,\lambda,\gamma)\propto g(\bmtheta,\lambda,\gamma) = e^{\lambda a(\bmtheta)+\gamma b(\bmtheta)}$. The gradient will be either with respect to $\lambda$ or $\gamma$ or both if they are equivalent. Hence,
\begin{align}
    \nabla\E_\rho[f(\bmtheta)]&=\nabla\lr{\frac{\int g(\bmtheta,\lambda,\gamma)f(\bmtheta)d\bmtheta}{\int g(\bmtheta,\lambda,\gamma)d\bmtheta. } }.%\\
    %&=\frac{\nabla \lr{\int g(\bmtheta,\lambda,\gamma)f(\bmtheta)d\bmtheta}}{\int g(\bmtheta,\lambda,\gamma)d\bmtheta } - \frac{\int g(\bmtheta,\lambda,\gamma)f(\bmtheta)d\bmtheta \nabla(\int g(\bmtheta,\lambda,\gamma)d\bmtheta) }{ (\int g(\bmtheta,\lambda,\gamma)d\bmtheta^2  }
\end{align}
Note that 
\begin{equation}
    \nabla g(\bmtheta,\lambda,\gamma) = \left\{\begin{array}{cc}
      a(\bmtheta)g(\bmtheta,\lambda,\gamma)   &  \mbox{ if }\lambda\neq\gamma\mbox{ , and gradient w.r.t. } \lambda \\
      b(\bmtheta)g(\bmtheta,\lambda,\gamma)   & \mbox{ if }\lambda\neq\gamma\mbox{ , and gradient w.r.t. } \gamma\\
      (a(\bmtheta)+b(\bmtheta))g(\bmtheta,\lambda,\gamma) & \mbox{ if }\lambda=\gamma=\tau \mbox{ , and gradient w.r.t. } \tau.
    \end{array} \right.
\end{equation}
Let $c(\bmtheta)$ denote $a(\bmtheta)$ if taking the gradient w.r.t. $\lambda$, 
denote $b(\bmtheta)$ if taking the gradient w.r.t. $\gamma$, and denote $a(\bmtheta)+b(\bmtheta)$ if $\lambda=\gamma=\tau$ and taking the gradient w.r.t. $\tau$. Then, the gradient of the Gibbs loss
\begin{equation}\label{eq:grad-gibbs-general}
    \nabla \E_\rho[f(\bmtheta)]=\E_\rho[c(\bmtheta)f(\bmtheta)]-\E_\rho[c(\bmtheta)]\E_\rho[f(\bmtheta)]=\mathbb{COV}_\rho(c(\bmtheta),f(\bmtheta)).
\end{equation}
\paragraph{Gradient of the Bayes loss} Next, we show a general result of the gradient of the Bayes loss, $\nabla B(\rho)$, for $\rho$ defined the same as above. By definition,
\begin{equation*}
    \nabla B(\rho) = \nabla \E_\nu\lrs{-\ln\E_\rho[p(\bmy|\bmx,\bmtheta)] } = -\E_\nu\lrs{\nabla \ln\E_\rho[p(\bmy|\bmx,\bmtheta) ] },
\end{equation*}
where
\begin{equation*}
    \nabla \ln\E_\rho[p(\bmy|\bmx,\bmtheta) ] = \frac{\nabla \E_\rho[p(\bmy|\bmx,\bmtheta)]}{\E_\rho[p(\bmy|\bmx,\bmtheta)]} = \frac{\mathbb{COV}_\rho(c(\bmtheta),p(\bmy|\bmx,\bmtheta)) }{\E_\rho[p(\bmy|\bmx,\bmtheta)]}
\end{equation*}
due to Eq.~\eqref{eq:grad-gibbs-general} for $f(\bmtheta)=p(\bmy|\bmx,\bmtheta)$ and $c(\bmtheta)$ follows the definition above. By expanding the covariance, the above formula further equals to
\begin{equation*}
    \frac{\E_\rho[c(\bmtheta)p(\bmy|\bmx,\bmtheta)]-\E_\rho[c(\bmtheta)]\E_\rho[p(\bmy|\bmx,\bmtheta)]}{\E_\rho[p(\bmy|\bmx,\bmtheta)]} = \E_{\tilde\rho}[c(\bmtheta)] - \E_\rho[c(\bmtheta)],
    %\frac{\E_\rho[c(\bmtheta)p(\bmy|\bmx,\bmtheta)]}{\E_\rho[p(\bmy|\bmx,\bmtheta)]} - \E_\rho[c(\bmtheta)].
\end{equation*}
%Put everything together, we have
%\begin{equation}\label{eq:grad-bayes-general}
%    \nabla B(\rho)=\E_\rho[c(\bmtheta)] - \E_\nu\lrs{\frac{\E_\rho[c(\bmtheta)p(\bmy|\bmx,\bmtheta)]}{\E_\rho[p(\bmy|\bmx,\bmtheta)]}} = \nabla B(\rho)=\E_\rho[c(\bmtheta)] - \E_{\bar \rho}[c(\bmtheta)].
%\end{equation}
where $\tilde\rho(\bmtheta|D,(\bmy,\bmx),\lambda,\gamma)\propto \rho(\bmtheta|D,\lambda,\gamma) p(\bmy|\bmx,\bmtheta)%=e^{\lambda a(\bmtheta)+\gamma b(\bmtheta)-\ell(\bmtheta)}
$, and $\ell(\bmtheta)$ is a shorthand of $\ell(\bmy|\bmx,\bmtheta)$. Put everything together, we have
\begin{equation}\label{eq:grad-bayes-general}
    \nabla B(\rho)=\E_\rho[c(\bmtheta)]-\E_\nu\E_{\tilde \rho}[c(\bmtheta)] = \E_\rho[c(\bmtheta)]-\E_{\bar \rho}[c(\bmtheta)],
\end{equation}
where \[\bar\rho(\bmtheta|D,\lambda,\gamma)=\E_\nu[\tilde \rho(\bmtheta|D,(\bmy,\bmx),\lambda,\gamma)]=\E_\nu\lrs{\frac{\rho(\bmtheta|D,\lambda,\gamma)p(\bmy|\bmx,\bmtheta)}{\E_{\rho}[p(\bmy|\bmx,\bmtheta)]}}.\] 
The last equality is because
\begin{align*}
    \E_\nu\E_{\tilde \rho}[c(\bmtheta)] &= \int_{(\bmy,\bmx)}\nu(\bmy,\bmx)\int_{\bmtheta} \tilde \rho (\bmtheta|D,(\bmy,\bmx),\lambda,\gamma) c(\bmtheta) d\bmtheta d(\bmy,\bmx)\\
    &=\int_\bmtheta \lr{\int_{(\bmy,\bmx)}\nu(\bmy,\bmx)\tilde\rho(\bmtheta|D,(\bmy,\bmx),\lambda,\gamma) d(\bmy,\bmx)} c(\bmtheta) d\bmtheta\\
    &=\int_\bmtheta \E_\nu [\tilde\rho(\bmtheta|D,(\bmy,\bmx),\lambda,\gamma)] c(\bmtheta) d\bmtheta\\
    &=\E_{\bar\rho}[c(\bmtheta)].
\end{align*}

\subsection{Likelihood Tempering Posterior}\label{app:sec:likelihoodTP}
We use the meta formulas to show the gradients of losses of likelihood-tempering posteriors. Recall that $p_\ell^\lambda(\bmtheta|D)\propto p(D|\bmtheta)^\lambda p(\bmtheta)=e^{-\lambda n \hat L(\bmtheta)+\ln p(\bmtheta)}$. Then, from Eq.~\eqref{eq:grad-gibbs-general}, we immediately obtain 
\[
\nabla_\lambda G(p_\ell^\lambda)=\nabla_\lambda \E_{p_\ell^\lambda}[L(\bmtheta)]=\mathbb{COV}_{p_\ell^\lambda}(-n\hat L(\bmtheta),L(\bmtheta))=-n\mathbb{COV}_{p_\ell^\lambda}(\hat L(\bmtheta),L(\bmtheta)),
\]
and
\[
\nabla_\lambda \hat G(p_\ell^\lambda)=\nabla_\lambda \E_{p_\ell^\lambda}[\hat L(\bmtheta)]=\mathbb{COV}_{p_\ell^\lambda}(-n\hat L(\bmtheta),\hat L(\bmtheta))=-n\mathbb{V}_{p_\ell^\lambda}(\hat L(\bmtheta)).
\]
On the other hand, by Eq.~\eqref{eq:grad-bayes-general}, we obtain
\[
\nabla_\lambda B(p_\ell^\lambda)=\E_{p_\ell^{\lambda}}[-n\hat L(\bmtheta)]-\E_{\bar p_\ell^\lambda}[-n\hat L(\bmtheta)]=-n\lr{\hat G(p_\ell^\lambda)-\hat G(\bar p_\ell^\lambda)},
\]
where 
\[
\bar p_\ell^\lambda(\bmtheta|D,(\bmy,\bmx),\lambda,\gamma)=\E_\nu\lrs{\frac{p_\ell^\lambda(\bmtheta|D)p(\bmy|\bmx,\bmtheta)}{\E_{p_\ell^\lambda}[p(\bmy|\bmx,\bmtheta)]}}. %\propto e^{-\lambda n\hat L(\bmtheta)+\ln p(\bmtheta)-\ell(\bmtheta)}
\]

\subsection{Prior Tempering Posterior}\label{app:sec:priorTP}
Recall that $p_\pi^\gamma(\bmtheta|D)\propto p(D|\bmtheta) p(\bmtheta)^\gamma=e^{- n \hat L(\bmtheta)+\gamma \ln p(\bmtheta)}$. Then, from Eq.~\eqref{eq:grad-gibbs-general}, we immediately obtain 
\[
\nabla_\gamma G(p_\pi^\gamma)=\nabla_\gamma \E_{p_\pi^\gamma}[L(\bmtheta)]=\mathbb{COV}_{p_\pi^\gamma}(\ln p(\bmtheta),L(\bmtheta)),
\]
and
\[
\nabla_\gamma \hat G(p_\pi^\gamma)=\nabla_\gamma \E_{p_\pi^\gamma}[\hat L(\bmtheta)]=\mathbb{COV}_{p_\pi^\gamma}(\ln p(\bmtheta),\hat L(\bmtheta)).
\]
On the other hand, by Eq.~\eqref{eq:grad-bayes-general}, we obtain
\[
\nabla_\lambda B(p_\pi^\gamma)=\E_{p_\pi^\gamma}[\ln p(\bmtheta)]-\E_{\bar p_\pi^\gamma}[\ln p(\bmtheta)],
\]
where 
\[\bar p_\pi^\gamma(\bmtheta|D,(\bmy,\bmx),\lambda,\gamma)=\E_\nu\lrs{\frac{p_\pi^\gamma(\bmtheta|D)p(\bmy|\bmx,\bmtheta)}{\E_{p_\pi^\gamma}[p(\bmy|\bmx,\bmtheta)]}}.
\]

\subsection{Full Tempering Posterior}\label{app:sec:fullTP}
Recall that $p_f^\tau(\bmtheta|D)\propto p(D|\bmtheta)^{\lambda=\tau} p(\bmtheta)^{\gamma=\tau}=e^{- \tau n \hat L(\bmtheta)+\tau \ln p(\bmtheta)}$. Then, from Eq.~\eqref{eq:grad-gibbs-general}, we have 
\begin{align*}
    \nabla_\tau G(p_f^\tau)&=\nabla_\tau \E_{p_f^\tau}[L(\bmtheta)]=\mathbb{COV}_{p_f^\tau}(-n\hat L(\bmtheta)+\ln p(\bmtheta),L(\bmtheta))\\
    &=-n\mathbb{COV}_{p_f^\tau}(\hat L(\bmtheta),L(\bmtheta))+\mathbb{COV}_{p_f^\tau}(\ln p(\bmtheta),L(\bmtheta)),
\end{align*}
and
\begin{align*}
    \nabla_\tau \hat G(p_f^\tau)&=\nabla_\tau \E_{p_f^\tau}[\hat L(\bmtheta)]=\mathbb{COV}_{p_f^\tau}(-n\hat L(\bmtheta)+\ln p(\bmtheta),\hat L(\bmtheta))\\
    &=-n\mathbb{V}_{p_f^\tau}(\hat L(\bmtheta))+\mathbb{COV}_{p_f^\tau}(\ln p(\bmtheta),\hat L(\bmtheta)).
\end{align*}
On the other hand, by Eq.~\eqref{eq:grad-bayes-general}, we obtain
\[
\nabla_\tau B(p_f^\tau)=\E_{p_f^\tau}[-n\hat L (\bmtheta)+\ln p(\bmtheta)]-\E_{\bar p_f^\tau}[-n\hat L(\bmtheta)+\ln p(\bmtheta)],
\]
where 
\[
\bar p_f^\tau(\bmtheta|D,(\bmy,\bmx),\lambda,\gamma)=\E_\nu\lrs{\frac{p_f^\tau(\bmtheta|D)p(\bmy|\bmx,\bmtheta)}{\E_{p_f^\tau}[p(\bmy|\bmx,\bmtheta)]}}.
\]

==> poster/definitions.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% COMMANDS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\ttt}{\texttt}

%%%%%%%%%%%%%% Proof
\newcommand{\bp}{\noindent{\emph{Proof}.}\ }
\newcommand{\ep}{\hfill $\Box$}

%%%%%%%%%%%%%% Equations
\newcommand{\BEAS}{\begin{eqnarray*}}
\newcommand{\EEAS}{\end{eqnarray*}}
\newcommand{\BEA}{\begin{eqnarray}}
\newcommand{\EEA}{\end{eqnarray}}
\newcommand{\BEQ}{\begin{equation}}
\newcommand{\EEQ}{\end{equation}}
\newcommand{\BIT}{\begin{itemize}}
\newcommand{\EIT}{\end{itemize}}
\newcommand{\BNUM}{\begin{enumerate}}
\newcommand{\ENUM}{\end{enumerate}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
\newcommand{\beqan}{\begin{eqnarray*}}
\newcommand{\eeqan}{\end{eqnarray*}}
\newcommand{\bealn}{\begin{align*}}
\newcommand{\eealn}{\end{align*}}
\newcommand{\al}[1]{ \begin{align} #1  \end{align}}
\newcommand{\eq}[1]{ \begin{equation} #1  \end{equation}}
\newcommand{\als}[1]{ \begin{align*} #1  \end{align*}}
\newcommand{\eqs}[1]{ \begin{equation*} #1  \end{equation*}}
\newcommand{\sk}{\nonumber\\}
\newcommand{\eqdef}{\stackrel{\textrm{def}}{=}}
\newcommand{\eqdefemph}{\stackrel{\textrm{\emph{def}}}{=}}
\def\NoNumber#1{{\def\alglinenumber##1{}\State #1}\addtocounter{ALG@line}{-1}}

%%%%%%%%%%%%%% Misc
\newcommand{\Lp}{\left(}
\newcommand{\Rp}{\right)}
\newcommand{\Lb}{\left[}
\newcommand{\Rb}{\right]}
\newcommand{\vs}{\vspace{0.2in}}
\newcommand{\hs}{\hspace{0.5in}}
\newcommand{\el}{\end{flushleft}}
\newcommand{\bl}{\begin{flushleft}}
\newcommand{\floor}[1]{  \lfloor #1 \rfloor}
\newcommand{\ceil}[1]{  \lceil #1 \rceil}
\newcommand{\inff}{\operatornamewithlimits{inf}}
\newcommand{\tto}[1]{\underset{#1}{\to}}
\newcommand{\eqdist}{\,{\buildrel d \over =}\,}
\renewcommand{\baselinestretch}{.98}
\newcommand{\iskip}{{\vskip -0.4cm}}
\newcommand{\siskip}{{\vskip -0.2cm}}
\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}
\newcommand{\argmin}{\arg\!\min}
\newcommand{\argmax}{\arg\!\max}
\newcommand{\Argmax}{\mathop{\mathrm{Argmax}}}

\newcommand{\bi}{ \begin{itemize} }
\newcommand{\ei}{ \end{itemize} }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MATH SYMBOLS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\bA}{\mathbb{A}}
\newcommand{\bB}{\mathbb{B}}
\newcommand{\bC}{\mathbb{C}}
\newcommand{\bD}{\mathbb{D}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\bF}{\mathbb{F}}
\newcommand{\bG}{\mathbb{G}}
\newcommand{\bH}{\mathbb{H}}
\newcommand{\bI}{\mathbb{I}}
\newcommand{\bJ}{\mathbb{J}}
\newcommand{\bK}{\mathbb{K}}
\newcommand{\bL}{\mathbb{L}}
\newcommand{\bM}{\mathbb{M}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\bO}{\mathbb{O}}
\newcommand{\bP}{\mathbb{P}}
\newcommand{\bQ}{\mathbb{Q}}
\newcommand{\bR}{\mathbb{R}}
\newcommand{\bS}{\mathbb{S}}
\newcommand{\bT}{\mathbb{T}}
\newcommand{\bU}{\mathbb{U}}
\newcommand{\bV}{\mathbb{V}}
\newcommand{\bW}{\mathbb{W}}
\newcommand{\bX}{\mathbb{X}}
\newcommand{\bY}{\mathbb{Y}}
\newcommand{\bZ}{\mathbb{Z}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\kA}{\mathfrak{A}}
\newcommand{\kB}{\mathfrak{B}}
\newcommand{\kC}{\mathfrak{C}}
\newcommand{\kD}{\mathfrak{D}}
\newcommand{\kE}{\mathfrak{E}}
\newcommand{\kF}{\mathfrak{F}}
\newcommand{\kG}{\mathfrak{G}}
\newcommand{\kH}{\mathfrak{H}}
\newcommand{\kI}{\mathfrak{I}}
\newcommand{\kJ}{\mathfrak{J}}
\newcommand{\kK}{\mathfrak{K}}
\newcommand{\kL}{\mathfrak{L}}
\newcommand{\kM}{\mathfrak{M}}
\newcommand{\kN}{\mathfrak{N}}
\newcommand{\kO}{\mathfrak{O}}
\newcommand{\kP}{\mathfrak{P}}
\newcommand{\kQ}{\mathfrak{Q}}
\newcommand{\kR}{\mathfrak{R}}
\newcommand{\kS}{\mathfrak{S}}
\newcommand{\kT}{\mathfrak{T}}
\newcommand{\kU}{\mathfrak{U}}
\newcommand{\kV}{\mathfrak{V}}
\newcommand{\kW}{\mathfrak{W}}
\newcommand{\kX}{\mathfrak{X}}
\newcommand{\kY}{\mathfrak{Y}}
\newcommand{\kZ}{\mathfrak{Z}}

\newcommand{\bsym}{\boldsymbol}
\newcommand{\Real}{\mathbb{R}}
\newcommand{\Nat}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\ind}{\mathbb{I}}
\newcommand{\indic}{\mathbb{I}}
\newcommand{\indOne}{\mathbbmss{1} }
\renewcommand{\phi}{\varphi}
\renewcommand{\epsilon}{\varepsilon}
%\renewcommand{\leq}{\leqslant}
%\renewcommand{\geq}{\geqslant}
%\renewcommand{\hat}{\widehat}

\def\M{{\mathbb M}}
\def\N{{\mathbb N}}
\def\NN{{\mathbb N}}
\def\EE{{\mathbb E}}
\def\PP{{\mathbb P}}
\def\RR{{\mathbb R}}
\def\ore{\overrightarrow{e}}
\def\orE{\overrightarrow{E}}
\def\ole{\overleftarrow{e}}
\def\d{\partial}
\def\bx{\bold{x}}
\def\bw{\bold{w}}
\def\bB{\bold{B}}
\def\Poi{\text{Poi}}
\def\Bin{\text{Bin}}
\def\odeg{\overline{\text{deg}}}
\def\Acal{{\mathcal A}}
\def\Pcal{{\mathcal P}}
\def\Rcal{{\mathcal R}}
\def\Dcal{{\mathcal D}}
\def\Ccal{{\mathcal C}}
\def\Ical{{\mathcal I}}
\def\Ocal{{\mathcal O}}
\def\Qcal{{\mathcal Q}}
\def\Bcal{{\mathcal B}}
\def\Hcal{{\mathcal H}}
\def\Ecal{{\mathcal E}}
\def\Fcal{{\mathcal F}}
\def\Ncal{{\mathcal N}}
\def\Mcal{{\mathcal M}}
\def\Lcal{{\mathcal L}}
\def\Kcal{{\mathcal K}}
\def\Gcal{{\mathcal G}}
\def\Scal{{\mathcal S}}
\def\Tcal{{\mathcal T}}
\def\Ucal{{\mathcal U}}
\def\Vcal{{\mathcal V}}
\def\Xcal{{\mathcal X}}
\def\Zcal{{\mathcal Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ABBREVIATIONS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\Span}{\bS}
\newcommand{\Esp}{\mathbb{E}}
\newcommand{\Var}{\mathbb{V}}
\newcommand{\var}{\mathbb{V}}
\renewcommand{\Pr}{\mathbb{P}}
\newcommand{\Normal}{\cN}
\newcommand{\Bern}{\mathrm{Ber}}
\newcommand{\bias}{b}
\newcommand{\Spanstar}{\Psi}
\newcommand{\supp}{\mathrm{supp}}
\newcommand{\llnp}{\mathrm{llnp}}
\newcommand{\kl}{\texttt{KL}}
\newcommand{\KL}{\texttt{KL}}
\newcommand{\klber}{\texttt{kl}}
\newcommand{\klg}{\texttt{KLG}}
\newcommand{\regret}{\mathfrak{R}}
\newcommand{\SP}{\textrm{SP}}

\newcommand{\ucb}{\textsc{\texttt{UCB1}}}
\newcommand{\klucb}{\textsc{\texttt{KL-UCB}}}
\newcommand{\TS}{\textsc{\texttt{TS}}}
\newcommand{\Ucrl}{\textsc{\texttt{Ucrl2}}}
\newcommand{\UCRL}{\textsc{\texttt{Ucrl2}}}
\newcommand{\KLUCRL}{\textsc{\texttt{KL-Ucrl}}}
%\newcommand{\BK}{\textsc{\texttt{Burnetas-Katehakis}}}
\newcommand{\BK}{\texttt{BK}}
\newcommand{\OLP}{\textsc{\texttt{OLP}}}
\newcommand{\regal}{\textsc{\texttt{Regal}}}
\newcommand{\QL}{\textsc{\texttt{Q-Learning}}}
\newcommand{\EVI}{\textsc{\texttt{Extended Value Iteration}}}
\newcommand{\geo}{\mathrm{geo}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MISC %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\setlength{\belowdisplayskip}{0pt}
\setlength{\abovedisplayskip}{0pt}
\setlength{\belowdisplayshortskip}{0pt}
\setlength{\abovedisplayshortskip}{0pt}



==> poster/packages.tex <==
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography

\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{bm}
\usepackage{bbm}
\usepackage{mathtools}
\usepackage{xspace}
\usepackage{wrapfig}
\usepackage{bookmark}

%\usepackage{times}
\usepackage{graphicx}

\newcommand{\subcaption}[1]% %1 = text
{\refstepcounter{subfig}%
\par\vskip\abovecaptionskip
\centerline{\textbf{(\alph{subfig})} #1}%
\vskip\belowcaptionskip\par}

% create subfigure environment
\def\subfigure{\let\oldcaption=\caption
\let\caption=\subcaption
\minipage}
\def\endsubfigure{\endminipage
\let\caption=\oldcaption}

\usepackage{algorithm}
\usepackage{algorithmic}

%----------------------------------
% For poster
%---------------------------------

\usepackage{xcolor}

\usepackage[framemethod=tikz, nobreak=true]{mdframed}



==> slides/beamer-preamble.tex <==
\mode<presentation>
{
  \usetheme{Tdn}
  % or ...

%  \setbeamercovered{transparent}
  \setbeamercovered{invisible}
  \usefonttheme{professionalfonts}
  % or whatever (possibly just delete it)
}

%\usepackage[english]{babel}
%\usepackage[latin1]{inputenc}
%\usepackage{times}
%\usepackage[T1]{fontenc}
%\usepackage{psfrag}
%\usepackage{amsmath}
%\usepackage{calc}
%\usepackage{ifthen}
%\usepackage{pifont}
%\usepackage{tdncolors}
%\usepackage{multirow}
%\usepackage{rotating}
%\usepackage{fancybox}
%\usepackage{ulem}
%\normalem


% Or whatever. Note that the encoding and the font should match. If T1
% does not look nice, try deleting the line with the fontenc.

\parindent 0mm

\include{macros}

\nc{\Subheading}[1]{\begin{center}{\bf\titleblue
      #1}\end{center}}

\nc{\Leftheading}[1]{{\bf\titleblue
      #1}}

\nc{\vsp}{\vspace{3mm}}
\nc{\texthighlight}{\schemeired}
\nc{\textnote}{\darkgreen}
%\nc{\boxhighlight}[2]{\psframebox*[fillcolor=#1]{#2}}
\nc{\boxhighlight}[2]{\colorbox{#1}{#2}}
\nc{\mystrut}[1]{\rule{0cm}{#1}}  % Used to control the height of a box

\nc{\var}[1]{{\titleblue #1}}
\nc{\st}[1]{{\texthighlight #1}}

\nc<>{\textmark}[1]{{\only#2{\textnote} {#1}}}


\newcommand\emphme[1]{%
	\ifmmode\text{\emph{#1}}\else\emph{#1}\fi%
}

\newenvironment{noteblock}[2][]{
\begin{beamerboxesrounded}[shadow=true]{#1}
#2}
{
\end{beamerboxesrounded}
}

\newenvironment{examblock}[2][]{
\begin{beamerboxesrounded}[shadow=true,lower=block body example,upper=block title example]{#1}
#2}
{
\end{beamerboxesrounded}
}


\AtBeginSection{
  \begin{center}
    \vspace*{30mm}
    \Large 
    {\color{titleblue}
    \insertsectionhead}
  \end{center}
}


\def\tlap#1{\vbox to0pt{\vss#1}}
\def\blap#1{\vbox to0pt{#1\vss}}
\def\clap#1{\hbox to 0pt{\hss#1\hss}}
\def\vclap#1{\vbox to 0pt{\vss#1\vss}}




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> slides/fancy.tex <==

\newcommand{\makenodes}{
    \Fovalnode[30mm]{5}{8}{Environment}{$E$: Environment}
    \Fovalnode[30mm]{2.5}{6.5}{Leak}{$L$: Leak}
    \Fovalnode[30mm]{7.5}{6.5}{GDfails}{$G$: GD failed}
    \Fovalnode[30mm]{5}{5}{Explosion}{$X$: Explosion}
    \Fovalnode[30mm]{5}{3.5}{Casualties}{$C$: Casualties}
}

\newcommand{\makeedges}{
    \arc{Environment}{Leak}
    \arc{Environment}{GDfails}
    \arc{Leak}{Explosion}
    \arc{GDfails}{Explosion}
    \arc{Explosion}{Casualties}
}



\newcommand{\influencediagram}{
%    \psset{linecolor=NTNUblue}
%    \psset{linewidth=2pt}
%
%    \Fovalnode[30mm]{5}{8}{Environment}{$E$: Environment}
%    \Fovalnode[30mm]{2.5}{6.5}{Leak}{$L$: Leak}
%    \Fovalnode[30mm]{7.5}{6.5}{GDfails}{$G$: GD failed}
%    \Fovalnode[30mm]{5}{5}{Explosion}{$X$: Explosion}
%    \Fovalnode[30mm]{5}{3.5}{Casualties}{$C$: Casualties}

    \psset{linecolor=black}
    \psset{linewidth=2pt}
    \makenodes
    \makeedges

    \psset{linecolor=MYgreen}
    \Frect[30mm]{14}{6.5}{NSSM}{SSM}
    \psset{linecolor=NTNUblue}
    \Fdiam[15mm]{14}{8}{NCost1}{Cost$_1$}
    \Fdiam[15mm]{5}{2}{NCost2}{Cost$_2$}

    \psset{linecolor=black}
    \arc{Environment}{NSSM}
\only<1>{\arc{NSSM}{Casualties}}
    \arc{NSSM}{Casualties}
    \arc{NSSM}{NCost1}
    \arc{Casualties}{NCost2}

    \only<2>{
        \Fovalnode[30mm]{14}{5}{Verification}{$F$: Effectiveness, SSM}

        \psset{linecolor=MYgreen}
        \Frect[30mm]{14}{3.5}{TAU}{Test interval}
        %\Frect[30mm]{14}{5}{TAU}{Test interval}

        \psset{linecolor=NTNUblue}
        \Fdiam[15mm]{14}{2}{NCost3}{Cost$_3$}
        %\Fdiam[15mm]{14}{3.5}{NCost3}{Cost$_3$}

        \psset{linecolor=black}
        \arc{NSSM}{Verification}
        \arc{Verification}{TAU}
        %\arc{NSSM}{TAU}
        \arc{TAU}{NCost3}
        \arc{TAU}{GDfails}
 %      \arc{Verification}{Casualties}
    }
}






\newcommand{\colorRed}{
    \psset{linecolor=red}
    \Fovalnode[30mm]{2.5}{6.5}{redLeak}{$L$: Leak}
    \Fovalnode[30mm]{7.5}{6.5}{redGDfails}{$G$: GD failed}
    \psset{linecolor=NTNUblue}
    \rput[lb](8, 4.5){\rnode{paDef}{\Red{$\pa{X}=\{L, G\}$}}}
    \psset{fillstyle=solid}\psset{fillcolor=lightgray}
    \Fovalnode[30mm]{5}{5}{Explosion}{$X$: Explosion}
    \psset{fillstyle=none} \psset{fillcolor=white}
}


\newcommand{\makeNonDescendants}{
    \psset{linecolor=MYgreen}
    \Fovalnode[30mm]{5}{8}{greenEnvironment}{$E$: Environment}
    \Fovalnode[30mm]{2.5}{6.5}{greenLeak}{$L$: Leak}
    \Fovalnode[30mm]{7.5}{6.5}{greenGDfails}{$G$: GD failed}
    \psset{linecolor=NTNUblue}
    \rput[lb](8, 3.8){\rnode{ndDef}{\Green{${\rm nd}(X)=\{E,L,G\}$}}}
}


\newcommand{\makeIndep}{
    \colorRed
%   \rput[lb](8, 3.1){\rnode{indepdDef}{$X \indep  \Green{E} \given \{\Red{L}, \Red{G}\}$ \big(Hence, $P(X\given \Green{E},\Red{L},\Red{G})=P(X\given \Red{L},\Red{G})$\big)}}
    \rput[lb](8, 3.1){\rnode{indepdDef}{$X \indep  \Green{E} \given \{\Red{L}, \Red{G}\}$}}
    \rput[lb](8, 2.4){\rnode{dSep}{\bf Other d-sep.\ rules: Jensen{\&}Nielsen (07)}} }


\newcommand{\makeCPT}{

%%% Get all nodes back to their original

    \psset{fillstyle=solid}\psset{fillcolor=white}
    \Fovalnode[30mm]{5}{5}{UnFilledExplosion}{$X$: Explosion}
    \psset{fillstyle=none} \psset{fillcolor=white}

    \makenodes % Get them back to original color
    \rput[lt](10.5,8.5){\rnode{CPT}{
    \begin{tabular}{lcc}\hline%\hline
    $G$ & $E=${\tt hostile} & $E=${\tt normal} \\
    \hline
    {\tt yes}   & $\lambda_H \cdot \tau/2$ & $\lambda_N\cdot\tau/2$ \\
    {\tt no}    & $1-\lambda_H\cdot\tau/2$ & $1-\lambda_N\cdot\tau/2$ \\
    \hline%\hline
    \end{tabular}
    }}

    \psset{linewidth=1pt}
    \psset{linecolor=black}
    \ncangle[angleA=-90,angleB=0,arm=.4cm,linestyle=dashed]{-}{CPT}{GDfails}
    \Aput{$P(G\given \Red{\pa{G}})$}

    \rput[lb](8, 3.1){\rnode{indepdDef}{\phantom{$X \indep  \Green{E} \given \{\Red{L}, \Red{G}\}$} \big(Hence, $P(X\given \Green{E},\Red{L},\Red{G})=P(X\given \Red{L},\Red{G})$\big)}}

%    \rput[lb](3, 1.8){$P(E, G, L, X, C) = P(E) P(G\given E) P(L\given E) $}
%    \rput[lb](6, 1.1){$\cdot ~~~P(X\given G, L) P(C\given X)$}


%   \rput[lb](3, 1.3){$P(E, L, G, X, C) = P(E) P(G\given E) P(L\given E)P(X\given G, L)P(C\given X)$}
    \rput[lb](3, 1.3){$P(E, L, G, X, C) = P(E)\cdot P(L\given \Red{E})\cdot P(G\given \Red{E}, \Green{L})  \cdot P(X\given \Green{E}, \Red{L}, \Red{G})  \cdot P(C\given \Green{E}, \Green{L}, \Green{G}, \Red{X})$}
    \rput[lb](5.9, 0.6){$               = P(E)\cdot P(L\given \Red{E})\cdot P(G\given \Red{E})\phantom{,L} \cdot P(X\given \Red{L}, \Red{G})\phantom{,E} \cdot P(C\given \Red{X})$}

%   \begin{eqnarray*}
%   P(E, G, L, X, C) & = & P(E) P(G\given E) P(L\given E, G) P(X\given E, G, L)P(C\given X, E, G, L)\\
%                    & = & P(E) P(G\given E) P(L\given E)P(X\given G, L)P(C\given X)\\
%   \end{eqnarray*}

}


\newcommand{\makeCausalStart}{%
\Fovalnode{17.7}{3.6}{NTTF1}{Effect}%
\Fovalnode{7.5}{3.6}{NCovariate1}{Cause}%
\arc{NCovariate1}{NTTF1}%
}%


\newcommand{\makeCausalConfounder}{
%    \psset{linecolor=red}{\red\Fovalnode{12.4}{7.2}{NConfounder}{Confounder}}\defaultLineColor
    \psset{linecolor=red}{\red\Fovalnode{12.3}{7.2}{NConfounder}{Management}}\defaultLineColor
    \Fovalnode{17.7}{3.6}{NTTF}{TTF}
    \Fovalnode{7.5}{3.6}{NCovariate}{Planned PM}
    \arc{NCovariate}{NTTF}
    \psset{linecolor=red}
    \dashedarc{NConfounder}{NCovariate}
    \dashedarc{NConfounder}{NTTF}
    \defaultLineColor
    \rput(12.1,1.7){\color{BrickRed}{NO! Destroyed by confounder}\defaultColor}
}



\newcommand{\makeCausalWorks}{
    \psset{linecolor=red}{\red\Fovalnode{12.4}{7.2}{NConfounder}{Management}}\defaultLineColor
    \Fovalnode{17.7}{3.6}{NTTF}{TTF}
    \Fovalnode{7.5}{3.6}{NCovariate}{Planned PM}
    \psset{linecolor=NTNUblue}\Fovalnode{12.6}{3.6}{NIntermediate}{\blue{Actual PM}}\defaultLineColor
    \psset{linecolor=NTNUblue}
    \arc{NIntermediate}{NTTF}\arc{NCovariate}{NIntermediate}
    \defaultLineColor

    \psset{linecolor=red}
    \dashedarc{NConfounder}{NCovariate}
    \dashedarc{NConfounder}{NTTF}
    \defaultLineColor
    \rput(12.1,1.7){\blue{Yes! Intermediate (observable) effect saves the
    day!}}


}



\newcommand{\makenodesInference}{
\Fnode{2}{6}{1N1}{$X_1$}      \Fnode{4}{6}{1N2}{$X_2$}
\Fnode{2}{4.5}{1N3}{$X_3$}    \Fnode{4}{4.5}{1N4}{$X_4$}
\Fnode{3}{2.5}{1N5}{$X_5$}%
%
%
\arc{1N1}{1N2} \arc{1N1}{1N3} \arc{1N2}{1N4} \arc{1N3}{1N5}
\arc{1N4}{1N5}

}






\nc{\moralInference}{


    \Fnode{6}{6}{2N1}{$X_1$}      \Fnode{8}{6}{2N2}{$X_2$}
    \Fnode{6}{4.5}{2N3}{$X_3$}    \Fnode{8}{4.5}{2N4}{$X_4$}
    \Fnode{7}{2.5}{2N5}{$X_5$}%


    \psset{linecolor=red}   \edge{2N3}{2N4}%
    \defaultLineColor

    \edge{2N1}{2N2} \edge{2N1}{2N3}
    \edge{2N2}{2N4} \edge{2N3}{2N5}
    \edge{2N4}{2N5}
}



\nc{\triangleInference}{


\Fnode{10}{6}{3N1}{$X_1$}      \Fnode{12}{6}{3N2}{$X_2$}
\Fnode{10}{4.5}{3N3}{$X_3$}    \Fnode{12}{4.5}{3N4}{$X_4$}
\Fnode{11}{2.5}{3N5}{$X_5$}%




% Skeleton
\edge{3N1}{3N2} \edge{3N1}{3N3} \edge{3N2}{3N4} \edge{3N3}{3N5}
\edge{3N4}{3N5}

%Moral part
\edge{3N3}{3N4}

% Triangulation

\psset{linecolor=green} \edge{3N1}{3N4}\defaultLineColor


}


\nc{\cliquesInference}{



\Fnode{14}{6}{4N1}{$X_1$}      \Fnode{16}{6}{4N2}{$X_2$}
\Fnode{14}{4.5}{4N3}{$X_3$}    \Fnode{16}{4.5}{4N4}{$X_4$}
\Fnode{15}{2.5}{4N5}{$X_5$}%


\psset{linecolor=lightgray}
% Skeleton
\edge{4N1}{4N2} \edge{4N1}{4N3} \edge{4N2}{4N4} \edge{4N3}{4N5}
\edge{4N4}{4N5}

%Moral part
\edge{4N3}{4N4}

% Triangulation
\edge{4N1}{4N4}


% Cliques
\pspolygon[linearc=.2cm,linecolor=blue](12.5,6.5)(16.5,6.5)(16.5,3.5)
\pspolygon[linearc=.2cm,linecolor=cyan](13.5,4.0)(13.5,7.0)(17.5,4.0)
\pspolygon[linearc=.2cm,linecolor=magenta](13.0,5.0)(17.0,5.0)(15.0,1.5)

\defaultLineColor

}






\nc{\joinTree}{


\psset{linecolor=magenta}\Fovalnode{3}{0.1}{Clique1}{$X_3$,$X_4$,$X_5$}\defaultLineColor
\psset{linecolor=cyan}\Fovalnode{9.5}{0.1}{Clique2}{$X_1$,$X_3$,$X_4$}\defaultLineColor
\psset{linecolor=NTNUblue}\Fovalnode{16}{0.1}{Clique3}{$X_1$,$X_2$,$X_4$}\defaultLineColor


\Fbox{6.25}{0}{Sep1}{$X_3$, $X_4$}
\Fbox{12.75}{0}{Sep2}{$X_1$,$X_4$}

\edge{Clique1}{Sep1}\edge{Sep1}{Clique2}\edge{Clique2}{Sep2}\edge{Sep2}{Clique3}


\rput(3.0,0.9){\scalebox{.7}{$\phi_1(x_3,x_4,x_5)$}}%
\rput(6.25,1.2){\scalebox{.7}{$\psi_1(x_3,x_4)$}}%
\rput(9.5,0.9){\scalebox{.7}{$\phi_2(x_1,x_3,x_4)$}}%
\rput(12.75,1.2){\scalebox{.7}{$\psi_2(x_1,x_4)$}}%
\rput(16,0.9){\scalebox{.7}{$\phi_3(x_1,x_2,x_4)$}}%
}


==> slides/hl_short.tex <==
\usepackage{xspace}
\usepackage{graphics,graphicx,epsfig}
\usepackage{url}

\newcommand{\nc}{\newcommand}

%      HELGE's EGNE "NEWCOMMANDS"



%%      THEOREMER OG SLIKT%
%
\newtheorem{hl_example}{Example}
\newtheorem{hl_algorithm}{Algorithm}
\newtheorem{hl_theorem}{Theorem}
\newtheorem{hl_proposition}{Proposition}
\newtheorem{hl_lemma}{Lemma}
\newtheorem{hl_corollary}{Corollary}
\newtheorem{hl_definition}{Definition}
\newtheorem{hl_conjecture}{Conjecture}
\newenvironment{hl_nonumberenv}[1]{{\bf #1}\begin{it}}{\end{it}}
\newtheorem{hl_proof}{Proof}



%      KOMMENTARMARKERING

\nc{\vekk}[1]{}   %         \vekk{Brukes for å markere vekk tekst}
%\nc{\comment}[1]{\mbox{}\marginpar{\raggedright\hspace{0pt}#1}}%
\nc{\hl}[1]{\comment{{\bf HL:} #1}} %
\nc{\tdn}[1]{\comment{{\bf TDN:} #1}} %



%      BEGIN/END

\nc{\bex}{\begin{example}} \nc{\eex}{\end{example}}

%\nc{\bth}{\begin{theorem}}
%\nc{\eth}{\end{theorem}}

\nc{\ble}{\begin{lemma}}
\nc{\ele}{\end{lemma}}

\nc{\bco}{\begin{conjecture}}
\nc{\eco}{\end{conjecture}}

\nc{\beq}{\begin{equation}}
\nc{\eeq}{\end{equation}}

\nc{\beqa}{\begin{eqnarray}}
\nc{\eeqa}{\end{eqnarray}}

\nc{\beqas}{\begin{eqnarray*}}%
\nc{\eeqas}{\end{eqnarray*}}

\nc{\bsp}{\[\begin{array}{rcl}}
\nc{\esp}{\end{array}\]}

\nc{\btab}[1]{\begin{tabular}{#1}}
\nc{\etab}{\end{tabular}}

\nc{\bfi}{\begin{figure}[htpb]}
\nc{\efi}{\end{figure}}

\nc{\ben}{\begin{enumerate}}
\nc{\een}{\end{enumerate}}

\nc{\bit}{\begin{itemize}}
\nc{\eit}{\end{itemize}}

\nc{\bde}{\begin{description}}
\nc{\ede}{\end{description}}


%      PRODUKT, BINOMISKE TING OG SUMMER

\nc{\pin}{\prod_{i=1}^n} \nc{\pjm}{\prod_{j=1}^m}
\nc{\pkm}{\prod_{k=1}^m} \nc{\pjM}{\prod_{j=1}^M}
\nc{\suin}{\sum_{i=1}^n} \nc{\sujm}{\sum_{j=1}^m}
\nc{\sukm}{\sum_{k=1}^m} \nc{\sujM}{\sum_{j=1}^M} \nc{\bimr}{\left
(_r^m \right)} \nc{\birs}{\left (_s^r \right)}
\nc{\bin}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%      CAL-TING
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\nc{\cal}{\mathcal}

\nc{\calDelta}{\mbox{$\cal{\Delta}$}}

% \nc{\calA}{\mbox{${\cal A}$}} \nc{\calB}{\mbox{$\cal{B}$}}
% \nc{\calC}{\mbox{$\cal{C}$}} \nc{\calD}{\mbox{$\cal{D}$}}
% \nc{\calE}{\mbox{$\cal{E}$}} \nc{\calF}{\mbox{$\cal{F}$}}
% \nc{\calG}{\mbox{$\cal{G}$}} \nc{\calH}{\mbox{$\cal{H}$}}
% \nc{\calI}{\mbox{$\cal{I}$}} \nc{\calJ}{\mbox{$\cal{J}$}}
% \nc{\calK}{\mbox{$\cal{K}$}} \nc{\calL}{\mbox{$\cal{L}$}}
% \nc{\calM}{\mbox{$\cal{M}$}} \nc{\calN}{\mbox{$\cal{N}$}}
% \nc{\calO}{\mbox{$\cal{O}$}} \nc{\calP}{\mbox{$\cal{P}$}}
% \nc{\calQ}{\mbox{$\cal{Q}$}} \nc{\calR}{\mbox{$\cal{R}$}}
% \nc{\calS}{\mbox{$\cal{S}$}} \nc{\calT}{\mbox{$\cal{T}$}}
% \nc{\calU}{\mbox{$\cal{U}$}} \nc{\calV}{\mbox{$\cal{V}$}}
% \nc{\calW}{\mbox{$\cal{W}$}} \nc{\calX}{\mbox{$\cal{X}$}}
% \nc{\calY}{\mbox{$\cal{Y}$}} \nc{\calZ}{\mbox{$\cal{Z}$}}
% \nc{\calz}{\mbox{$\cal{z}$}}



\nc{\calA}{{\ensuremath{\cal{A}}}} \nc{\calB}{{\ensuremath{\cal{B}}}}
\nc{\calC}{{\ensuremath{\cal{C}}}} \nc{\calD}{{\ensuremath{\cal{D}}}}
\nc{\calE}{{\ensuremath{\cal{E}}}} \nc{\calF}{{\ensuremath{\cal{F}}}}
\nc{\calG}{{\ensuremath{\cal{G}}}} \nc{\calH}{{\ensuremath{\cal{H}}}}
\nc{\calI}{{\ensuremath{\cal{I}}}} \nc{\calJ}{{\ensuremath{\cal{J}}}}
\nc{\calK}{{\ensuremath{\cal{K}}}} \nc{\calL}{{\ensuremath{\cal{L}}}}
\nc{\calM}{{\ensuremath{\cal{M}}}} \nc{\calN}{{\ensuremath{\cal{N}}}}
\nc{\calO}{{\ensuremath{\cal{O}}}} \nc{\calP}{{\ensuremath{\cal{P}}}}
\nc{\calQ}{{\ensuremath{\cal{Q}}}} \nc{\calR}{{\ensuremath{\cal{R}}}}
\nc{\calS}{{\ensuremath{\cal{S}}}} \nc{\calT}{{\ensuremath{\cal{T}}}}
\nc{\calU}{{\ensuremath{\cal{U}}}} \nc{\calV}{{\ensuremath{\cal{V}}}}
\nc{\calW}{{\ensuremath{\cal{W}}}} \nc{\calX}{{\ensuremath{\cal{X}}}}
\nc{\calY}{{\ensuremath{\cal{Y}}}} \nc{\calZ}{{\ensuremath{\cal{Z}}}}
\nc{\calz}{{\ensuremath{\cal{z}}}}



%\nc{\NP}{\mbox{$\calN\calP$}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%      BOLDMATH-TING
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\nc{\bm}{\boldmath}
% \nc{\bm}{\bf}
\nc{\bma}{{\ensuremath{\boldsymbol{a}}}} 
\nc{\bmb}{{\ensuremath{\boldsymbol{b}}}}
\nc{\bmc}{{\ensuremath{\boldsymbol{c}}}} \nc{\bmd}{{\ensuremath{\boldsymbol{d}}}}
\nc{\bme}{{\ensuremath{\boldsymbol{e}}}} \nc{\bmf}{{\ensuremath{\boldsymbol{f}}}}
\nc{\bmg}{{\ensuremath{\boldsymbol{g}}}} \nc{\bmh}{{\ensuremath{\boldsymbol{h}}}}
\nc{\bmi}{{\ensuremath{\boldsymbol{i}}}} \nc{\bmj}{{\ensuremath{\boldsymbol{j}}}}
\nc{\bmk}{{\ensuremath{\boldsymbol{k}}}} \nc{\bml}{{\ensuremath{\boldsymbol{l}}}}
\nc{\bmm}{{\ensuremath{\boldsymbol{m}}}} \nc{\bmn}{{\ensuremath{\boldsymbol{n}}}}
\nc{\bmo}{{\ensuremath{\boldsymbol{o}}}} \nc{\bmp}{{\ensuremath{\boldsymbol{p}}}}
\nc{\bmq}{{\ensuremath{\boldsymbol{q}}}} \nc{\bmr}{{\ensuremath{\boldsymbol{r}}}}
\nc{\bms}{{\ensuremath{\boldsymbol{s}}}} \nc{\bmt}{{\ensuremath{\boldsymbol{t}}}}
\nc{\bmu}{{\ensuremath{\boldsymbol{u}}}} \nc{\bmv}{{\ensuremath{\boldsymbol{v}}}}
\nc{\bmw}{{\ensuremath{\boldsymbol{w}}}} \nc{\bmx}{{\ensuremath{\boldsymbol{x}}}}
\nc{\bmy}{{\ensuremath{\boldsymbol{y}}}} \nc{\bmz}{{\ensuremath{\boldsymbol{z}}}}

% \nc{\bma}{{\mbox{\bm $a$}}} 
% \nc{\bmb}{{\mbox{\bm $b$}}}
% \nc{\bmc}{{\mbox{\bm $c$}}} \nc{\bmd}{{\mbox{\bm $d$}}}
% \nc{\bme}{{\mbox{\bm $e$}}} \nc{\bmf}{{\mbox{\bm $f$}}}
% \nc{\bmg}{{\mbox{\bm $g$}}} \nc{\bmh}{{\mbox{\bm $h$}}}
% \nc{\bmi}{{\mbox{\bm $i$}}} \nc{\bmj}{{\mbox{\bm $j$}}}
% \nc{\bmk}{{\mbox{\bm $k$}}} \nc{\bml}{{\mbox{\bm $l$}}}
% \nc{\bmm}{{\mbox{\bm $m$}}} \nc{\bmn}{{\mbox{\bm $n$}}}
% \nc{\bmo}{{\mbox{\bm $o$}}} \nc{\bmp}{{\mbox{\bm $p$}}}
% \nc{\bmq}{{\mbox{\bm $q$}}} \nc{\bmr}{{\mbox{\bm $r$}}}
% \nc{\bms}{{\mbox{\bm $s$}}} \nc{\bmt}{{\mbox{\bm $t$}}}
% \nc{\bmu}{{\mbox{\bm $u$}}} \nc{\bmv}{{\mbox{\bm $v$}}}
% \nc{\bmw}{{\mbox{\bm $w$}}} \nc{\bmx}{{\mbox{\bm $x$}}}
% \nc{\bmy}{{\mbox{\bm $y$}}} \nc{\bmz}{{\mbox{\bm $z$}}}


\nc{\bmA}{{\ensuremath{\boldsymbol{A}}}} \nc{\bmB}{{\ensuremath{\boldsymbol{B}}}}
\nc{\bmC}{{\ensuremath{\boldsymbol{C}}}} \nc{\bmD}{{\ensuremath{\boldsymbol{D}}}}
\nc{\bmE}{{\ensuremath{\boldsymbol{E}}}} \nc{\bmF}{{\ensuremath{\boldsymbol{F}}}}
\nc{\bmG}{{\ensuremath{\boldsymbol{G}}}} \nc{\bmH}{{\ensuremath{\boldsymbol{H}}}}
\nc{\bmI}{{\ensuremath{\boldsymbol{I}}}} \nc{\bmJ}{{\ensuremath{\boldsymbol{J}}}}
\nc{\bmK}{{\ensuremath{\boldsymbol{K}}}} \nc{\bmL}{{\ensuremath{\boldsymbol{L}}}}
\nc{\bmM}{{\ensuremath{\boldsymbol{M}}}} \nc{\bmN}{{\ensuremath{\boldsymbol{N}}}}
\nc{\bmO}{{\ensuremath{\boldsymbol{O}}}} \nc{\bmP}{{\ensuremath{\boldsymbol{P}}}}
\nc{\bmQ}{{\ensuremath{\boldsymbol{Q}}}} \nc{\bmR}{{\ensuremath{\boldsymbol{R}}}}
\nc{\bmS}{{\ensuremath{\boldsymbol{S}}}} \nc{\bmT}{{\ensuremath{\boldsymbol{T}}}}
\nc{\bmU}{{\ensuremath{\boldsymbol{U}}}} \nc{\bmV}{{\ensuremath{\boldsymbol{V}}}}
\nc{\bmW}{{\ensuremath{\boldsymbol{W}}}} \nc{\bmX}{{\ensuremath{\boldsymbol{X}}}}
\nc{\bmY}{{\ensuremath{\boldsymbol{Y}}}} \nc{\bmZ}{{\ensuremath{\boldsymbol{Z}}}}

% \nc{\bmA}{{\mbox{\bm $A$}}} \nc{\bmB}{{\mbox{\bm $B$}}}
% \nc{\bmC}{{\mbox{\bm $C$}}} \nc{\bmD}{{\mbox{\bm $D$}}}
% \nc{\bmE}{{\mbox{\bm $E$}}} \nc{\bmF}{{\mbox{\bm $F$}}}
% \nc{\bmG}{{\mbox{\bm $G$}}} \nc{\bmH}{{\mbox{\bm $H$}}}
% \nc{\bmI}{{\mbox{\bm $I$}}} \nc{\bmJ}{{\mbox{\bm $J$}}}
% \nc{\bmK}{{\mbox{\bm $K$}}} \nc{\bmL}{{\mbox{\bm $L$}}}
% \nc{\bmM}{{\mbox{\bm $M$}}} \nc{\bmN}{{\mbox{\bm $N$}}}
% \nc{\bmO}{{\mbox{\bm $O$}}} \nc{\bmP}{{\mbox{\bm $P$}}}
% \nc{\bmQ}{{\mbox{\bm $Q$}}} \nc{\bmR}{{\mbox{\bm $R$}}}
% \nc{\bmS}{{\mbox{\bm $S$}}} \nc{\bmT}{{\mbox{\bm $T$}}}
% \nc{\bmU}{{\mbox{\bm $U$}}} \nc{\bmV}{{\mbox{\bm $V$}}}
% \nc{\bmW}{{\mbox{\bm $W$}}} \nc{\bmX}{{\mbox{\bm $X$}}}
% \nc{\bmY}{{\mbox{\bm $Y$}}} \nc{\bmZ}{{\mbox{\bm $Z$}}}




\nc{\bmUpsilon}{{\mbox{\bm $\boldsymbol{\Upsilon}$}}}
\nc{\bmupsilon}{{\mbox{\bm $\boldsymbol{\upsilon}$}}}
\nc{\bmalpha}{{\mbox{\bm $\boldsymbol{\alpha}$}}}
\nc{\bmbeta}{{\mbox{\bm $\boldsymbol{\beta}$}}}
\nc{\bmgamma}{{\mbox{\bm $\boldsymbol{\gamma}$}}}
\nc{\bmGamma}{{\mbox{\bm $$\boldsymbol{\Gamma}$}}}
\nc{\bmdelta}{{\mbox{\bm $\boldsymbol{\delta}$}}}
\nc{\bmDelta}{{\mbox{\bm $\boldsymbol{\Delta}$}}}
\nc{\bmeps}{{\mbox{\bm $\boldsymbol{\epsilon}$}}}
\nc{\bmepsilon}{\bmeps}
\nc{\bmphi}{{\mbox{\bm $\boldsymbol{\phi}$}}}
\nc{\bmPhi}{{\mbox{\bm $\$\boldsymbol{\Phi}$}}}
\nc{\bmlambda}{{\mbox{\bm $\boldsymbol{\lambda}$}}}
\nc{\bmLambda}{{\mbox{\bm $\boldsymbol{\Lambda}$}}}
\nc{\bmmu}{{\mbox{\bm $\boldsymbol{\mu}$}}}
\nc{\bmnu}{{\mbox{\bm $\boldsymbol{\nu}$}}}
\nc{\bmpi}{{\mbox{\bm $\boldsymbol{\pi}$}}}
\nc{\bmrho}{{\mbox{\bm$\boldsymbol{\rho}$}}}
\nc{\bmpsi}{{\mbox{\bm $\boldsymbol{\psi}$}}}
\nc{\bmPsi}{{\mbox{\bm $\boldsymbol{\Psi}$}}}
\nc{\bmsigma}{{\mbox{\bm $$\boldsymbol{\sigma}$}}}
\nc{\bmSigma}{{\mbox{\bm $\boldsymbol{\Sigma}$}}}
\nc{\bmtheta}{{\ensuremath{\boldsymbol{\theta}}}}
%\nc{\bmTheta}{{\mbox{\bm $\Theta$}}}
\nc{\bmTheta}{{\ensuremath{\boldsymbol{\Theta}}}}
\nc{\bmeta}{{\ensuremath{\boldsymbol{\eta}}}}
\nc{\bmzeta}{{\mbox{\bm $\zeta$}}}
\nc{\bmxi}{{\mbox{\bm $\xi$}}} \nc{\bmXi}{{\mbox{\bm $\Xi$}}}
\nc{\bmnabla}{{\mbox{\bm $\nabla$}}}
\nc{\bmomega}{{\mbox{\bm $\omega$}}}
\nc{\bmOmega}{{\mbox{\bm $\Omega$}}}

\nc{\bmen}{{\bf 1}} \nc{\bmhalf}{{\bf\frac{1}{2}}}
\nc{\bmnull}{{\bf \ensuremath{0}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% General terminology
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nc{\Var}{\mbox{Var}} \nc{\Cov}{\mbox{Cov}}
\nc{\E}{\mbox{$\mathbb{E}$}}
\nc{\KL}[2]{D\left(\,#1\,\norm\,#2\,\right)}
\nc{\convL}{\stackrel{\calL}{\rightarrow}} \nc{\given}{|}
%\nc{\norm}{||}
\nc{\norm}{\|} \nc{\sizeof}[1]{\left|#1\right|}

\nc{\iffp}{\mbox{$\Leftrightarrow$}} \nc{\ien}{\mbox{$i=1\ld n$}}
%\nc{\R}{\mbox{$\mathbb{R}$}}
\nc{\nat}{\mbox{$\mathbb{N}$}} \nc{\infinity}{\infty}
\nc{\ld}{,\ldots,} \nc{\defi}{:=} \nc{\incl}{\subset}
\nc{\upin}[2]{#1^{(#2)}} \nc{\non}{\nonumber}
\nc{\stless}{\stackrel{\mbox{st}}{\leq}}
\gdef\qed{\relax\ifmmode~\hfill\square\else\unskip\nobreak
    ~\hfill$\square$\fi}
\nc{\boxen}{\begin{flushright}$\rule{3mm}{3mm}$\end{flushright}}
\newcommand{\trans}{^{\mbox{\tiny{T}}}}
%\newcommand{\trans}{\top}
\newcommand{\T}{\trans}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Special reliability analysis
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nc{\h}{\mbox{$h(\bmp)$}}
\nc{\hm}{\mbox{$h^m(\bmp)$}}
\nc{\hnei}{\mbox{$h({\bf p})$}}
\nc{\hmnei}{\mbox{$h^m({\bf p})$}}
\nc{\hj}{h_j(\bmp)}
\nc{\hmj}{h_j^m(\bmp)}
\nc{\hjm}{\hmj}
\nc{\ph}{\phi(\bmx)}
\nc{\Ph}{\phi(\bmX)}
%\nc{\p}{\overline P}
\nc{\ip}{\coprod}
\nc{\phd}{\phi^D (\bmx)}
\nc{\Phd}{\phi^D(\bmX)}
\nc{\hd}{h^D (\bmp)}
\nc{\hdm}{\left( h^D (\bmp) \right)^m}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BN related stuff
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \nc{\pa}[1]{{\rm pa}\left(#1\right)}
 \nc{\mb}[1]{{\rm mb}\left(#1\right)}
 \nc{\sspace}[1]{\ensuremath{sp\left(#1\right)}}
% \nc{\sspace}[1]{{\rm sp}\left(#1\right)}
 \nc{\child}[1]{\mbox{${\rm ch}\left(#1\right)$}}
 \nc{\indep}{\mbox{$\perp\!\!\!\perp$}}
 \nc{\nonindep}{\not\!\!\!\indep} \nc{\NB}{Na\"{\i}ve Bayes\xspace}
 \nc{\nB}{na\"{\i}ve Bayes\xspace}
 \nc{\MDL}{\mbox{MDL}\xspace} \nc{\MDLp}{$\mbox{MDL}_p$\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This part here for the HuginToPsTrics stuff by Thomas
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Fbox}[5][0.5cm]{\rput(#2,#3){\rnode{#4}{\psframebox{\parbox[c][#1]{#1}{\centerline{#5}}}}}}
\newcommand{\Fnode}[5][0.5cm]{\cnodeput[doubleline=false](#2,#3){#4}{\makebox[#1]{#5}}}
\newcommand{\FDblnode}[5][0.5cm]{\cnodeput[doubleline=true](#2,#3){#4}{\makebox[#1]{#5}}}
\newcommand{\Fdiam}[5][0.3cm]{\rput(#2,#3){\dianode{#4}{\makebox[#1]{#5}}}}
\newcommand{\Fovalnode}[5][0.5cm]{\rput(#2,#3){\ovalnode{#4}{\makebox[#1]{#5}}}}
\newcommand{\FDblovalnode}[5][0.5cm]{\rput(#2,#3){\ovalnode[doubleline=true]{#4}{\makebox[#1]{#5}}}}
\newcommand{\Frect}[5][0.5cm]{\rput(#2,#3){\rnode{#4}{\psframebox{\makebox[#1]{#5}}}}}
\newcommand{\arc}[3][solid]{\ncline[linestyle=#1]{->}{#2}{#3}}
%\newpsobject{showgrid}{psgrid}{subgriddiv=1,griddots=10,gridlabels=6pt}
%\psset{unit=0.5cm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% pstexfig: Latex-type figures from xfig.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\pstexfig}[2] {
\begin{nopagebreak}
  \begin{figure}[htpb]
    \begin{center}
      \input{./FIGS/#1.pstex_t}
        \caption{#2}
      \label{fig:#1}
    \end{center}
  \end{figure}
\end{nopagebreak}
}

\newcommand{\pstexFig}[2] {
\begin{nopagebreak}
  \begin{figure*}[htbp]
    \begin{center}
      \input{./FIGS/#1.pstex_t}
        \caption{#2}
      \label{fig:#1}
    \end{center}
  \end{figure*}
\end{nopagebreak}
}

\newcommand{\pstexfigSlide}[1] {
\begin{nopagebreak}
    \begin{center}
        \input{./#1.pstex_t}
    \end{center}
\end{nopagebreak}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% epsfigur: Get an eps-fig from file
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\epsfigur}[3] {
\begin{nopagebreak}
  \begin{figure}[htpb]
    \begin{center}
      \epsfig{file =./FIGS/#1.eps,width=#3mm}
        \caption{#2}
      \label{fig:#1}
    \end{center}
  \end{figure}
\end{nopagebreak}
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% psfigur: Get an ps-fig from file
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\psfigur}[3] {
\begin{nopagebreak}
  \begin{figure}[htpb]
    \begin{center}
      \psfig{file =./FIGS/#1.ps,width=#3mm,angle=-90}
       \caption{#2}
      \label{fig:#1}
    \end{center}
  \end{figure}
\end{nopagebreak}
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Rpsfigur: Get an ps-fig from file
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Rpsfigur}[3] {
\begin{nopagebreak}
  \begin{figure}[htpb]
    \begin{center}
      \psfig{file =./FIGS/#1.ps,width=#3mm}
       \caption{#2}
      \label{fig:#1}
    \end{center}
  \end{figure}
\end{nopagebreak}
}



\nc{\figref}[1]{\figurename~\ref{fig:#1}\xspace}
\nc{\tabref}[1]{Table~\ref{tab:#1}\xspace}
\nc{\equref}[1]{Equation~(\ref{equ:#1})\xspace}
\nc{\secref}[1]{Section~\ref{sec:#1}\xspace}
\nc{\algoref}[1]{Algorithm~\ref{algo:#1}\xspace}
\nc{\stepref}[1]{Step~\ref{step:#1}\xspace}

\nc{\includebib}{\bibliography{defs,%
                               hl,%
                               master,%
                               dynamic,%
                               reliability,%
                               troubleshoot,%
                               class,%
                               learning,%
                               luigi,%
			      footy,%
                               antonio,%
%                               mte,%
                               global%
}}


==> slides/macros.tex <==
%\usepackage{xspace}
%\usepackage{ifthen}

\newcommand{\nc}{\newcommand}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% Setup stuff
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\nc{\corref}[2][]{\corollaryname~\ref{cor:#2}\ifthenelse{\equal{#1}{}}{}{(#1)}\xspace}
\nc{\defref}[2][]{\definitionname~\ref{def:#2}\ifthenelse{\equal{#1}{}}{}{(#1)}\xspace}
\nc{\figref}[2][]{\figurename~\ref{fig:#2}\ifthenelse{\equal{#1}{}}{}{(#1)}\xspace}
\nc{\thmref}[2][]{\theoremname~\ref{thm:#2}\ifthenelse{\equal{#1}{}}{}{(#1)}\xspace}
\nc{\tabref}[2][]{\tablename~\ref{tab:#2}\ifthenelse{\equal{#1}{}}{}{(#1)}\xspace}
\nc{\exaref}[2][]{\examplename~\ref{exa:#2}\ifthenelse{\equal{#1}{}}{}{(#1)}\xspace}
\nc{\equref}[1]{\equationname~\ref{equ:#1}\xspace}
\nc{\secref}[1]{\sectionname~\ref{#1}\xspace}
\nc{\charef}[1]{\chaptername~\ref{cha:#1}\xspace}
\nc{\proref}[1]{\propositionname~\ref{pro:#1}\xspace}
%\nc{\algref}[1]{\algorithmname~\ref{alg:#1}\xspace}
\nc{\exeref}[1]{\exercisename~\ref{exe:#1}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% Color related stuff
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\nc{\Blue}[1]{\begin{blue}#1\end{blue}}
\nc{\Red}[1]{\begin{red}#1\end{red}}
\nc{\Green}[1]{\begin{green}#1\end{green}}
\nc{\Purple}[1]{\begin{magenta}#1\end{magenta}}
%\nc{\Black}[1]{\begin{black}#1\end{black}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% Misc stuff
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
\nc{\ul}[1]{\underline{#1}}
\nc{\bm}{\mathbf}
%\nc{\cal}{\mathcal}
\providecommand{\cal}{\mathcal}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% Debugging stuff
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newboolean{DEBUG}

%\newboolean{COMMENT}
%\nc{\comment}[1]{\ifthenelse{\boolean{COMMENT}}{\vspace*{0.5cm}\noindent
%\framebox[\linewidth][l]{\begin{minipage}{0.95\linewidth}{\bf Comment:} #1\end{minipage}}
%\newline}{}}

%\nc{\debug}[1]{\ifthenelse{\equal{\DEBUG}{1}}{\framebox[\linewidth][l]{{\bf Debug:} #1\hfill}\newline}{}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% General stuff
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\nc{\trans}{^{\mbox{\tiny{T}}}}
\nc{\T}{\trans}
\nc{\set}{\cal}
\nc{\true}{\ensuremath{\mathrm{true}}}
\nc{\false}{\ensuremath{\mathrm{false}}}
\nc{\score}{\mathop{\mathrm{score}}}
\nc{\grad}{\mathop{\mathrm{\bm{grad}}}}
\nc{\dist}{\mathop{\mathrm{dist}}}
\nc{\reals}{\ensuremath{\mathbb{R}}}
\nc{\cardinal}[1]{\mathopen{|}#1\mathclose{|}}
\nc{\Nset}{\mathbb N}
\nc{\Zset}{\mathbb Z}
\nc{\Rset}{\mathbb R}
\nc{\Qset}{\mathbb Q}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% Pstricks stuff
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \nc{\Fbox}[5][0.5cm]{\rput(#2,#3){\rnode{#4}{\psframebox{\parbox[c][#1]{#1}{\centerline{#5}}}}}}
% \nc{\Fnode}[5][0.5cm]{\cnodeput[doubleline=false](#2,#3){#4}{\makebox[#1]{#5}}}
% \nc{\FDblnode}[5][0.5cm]{\cnodeput(#2,#3){#4}{\makebox[#1]{#5}}}
% \nc{\Fdiam}[5][0.3cm]{\rput(#2,#3){\dianode{#4}{\makebox[#1]{#5}}}}
% \nc{\Fovalnode}[5][0.5cm]{\rput(#2,#3){\ovalnode{#4}{\makebox[#1]{#5}}}}
% \nc{\FDblovalnode}[5][0.5cm]{\rput(#2,#3){\ovalnode[doubleline=true]{#4}{\makebox[#1]{#5}}}}
% \nc{\Frect}[5][0.5cm]{\rput(#2,#3){\rnode{#4}{\psframebox{\makebox[#1]{#5}}}}}
% \nc{\arc}[3][solid]{\ncline[linestyle=#1]{->}{#2}{#3}}
% %\psset{unit=0.5cm}
% \newpsobject{showgrid}{psgrid}{subgriddiv=1,griddots=10,gridlabels=6pt}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% Bayesian network related stuff
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\nc{\BIC}{\ensuremath{\mathrm{BIC}}\xspace}
\nc{\MDL}{\ensuremath{\mathrm{MDL}}\xspace}
\nc{\Dir}{\ensuremath{\mathrm{Dir}}\xspace}
\nc{\f}{P^{\#}}
\nc{\Var}{\mathop{\rm Var}}
\nc{\MPE}{\mathop{\rm MPE}}
\nc{\MAP}{\mathop{\rm MAP}}
\nc{\Cov}{\mathop{\rm Cov}}
\nc{\MI}{\mathop{\rm MI}}
\nc{\CMI}{\mathop{\rm CMI}}
\nc{\KL}{\mathop{\rm KL}}
\nc{\KLd}[2]{\KL\left(#1||#2\right)}
\nc{\ent}{\mathop{\rm Ent}}
\nc{\given}{\,|\,}
\nc{\Exp}{\mathop{\mathbb{E}}}
\nc{\indep}{\mathrel{\perp\!\!\!\perp}}
\nc{\nonindep}{\mathrel{\not\!\!\!\perp\!\!\!\perp}}
\nc{\NB}{Naive Bayes\xspace}
\nc{\nB}{naive Bayes\xspace}
%\nc{\sspace}[1]{\mathop{\mathrm{sp}\left(#1\right)}}
\nc{\sspace}[1]{\mathop{\mathrm{sp}(#1)}}
\nc{\sizeof}[1]{\left|#1\right|}
\nc{\conf}{\mathop{\mathrm{conf}}}
%\nc{\pa}[1]{\mathop{\mathrm{pa}}\left\mathopen(#1\right\mathclose)}

\nc{\pa}[1]{\mathop{\mathrm{pa}}(#1)}
\nc{\ch}[1]{\mathop{\mathrm{ch}}(#1)}
\nc{\fa}[1]{\mathop{\mathrm{fa}}(#1)}
\nc{\nb}[1]{\mathop{\mathrm{nb}}(#1)}
\nc{\nd}[1]{\mathop{\mathrm{nd}}(#1)}

% \nc{\pa}[1]{\mathop{\mathrm{pa}}\left(#1\right)}
% \nc{\ch}[1]{\mathop{\mathrm{ch}}\left(#1\right)}
% \nc{\fa}[1]{\mathop{\mathrm{fa}}\left(#1\right)}
% \nc{\nb}[1]{\mathop{\mathrm{nb}}\left(#1\right)}
\nc{\dom}[1]{\mathop{\mathrm{dom}}\left(#1\right)}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% Influence diagram related stuff
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\nc{\past}[1]{\mathop{\rm past}(#1 )}
\nc{\pred}[1]{\mathop{\rm pred}(#1 )}
\nc{\req}[1]{\mathop{\rm req} (#1 )}
% \nc{\past}[1]{\mathop{\rm past}\left (#1\right )}
% \nc{\pred}[1]{\mathop{\rm pred}\left (#1\right )}
% \nc{\req}[1]{\mathop{\rm req}\left (#1\right )}
\nc{\strategy}{\Delta}		
\nc{\policy}{\delta}		
\nc{\eu}{\ensuremath{\mathop{\rm EU}}}		
\nc{\meu}{\mathop{\rm MEU}}		
%\nc{\meu}{\mbox{\emph{MEU}}}		


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% Planning under uncertainty
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\nc{\MDP}{MDP\xspace}
\nc{\POMDP}{POMDP\xspace}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% Troubleshooting
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\nc{\ECR}{\mathop{\mathrm{ECR}}\xspace}
\nc{\ef}{\mathop{\mathrm{ef}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% Boldmath stuff
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\nc{\bma}{{\mbox{\bm $a$}}}
\nc{\bma}{\mathalpha{\bm a}}
\nc{\bmb}{\mathalpha{\bm b}}
\nc{\bmc}{\mathalpha{\bm c}}
\nc{\bmd}{\mathalpha{\bm d}}
\nc{\bme}{\mathalpha{\bm e}}
\nc{\bmf}{\mathalpha{\bm f}}
\nc{\bmg}{\mathalpha{\bm g}}
\nc{\bmh}{\mathalpha{\bm h}}
\nc{\bmi}{\mathalpha{\bm i}}
\nc{\bmj}{\mathalpha{\bm j}}
\nc{\bmk}{\mathalpha{\bm k}}
\nc{\bml}{\mathalpha{\bm l}}
\nc{\bmm}{\mathalpha{\bm m}}
\nc{\bmn}{\mathalpha{\bm n}}
\nc{\bmo}{\mathalpha{\bm o}}
\nc{\bmp}{\mathalpha{\bm p}}
\nc{\bmq}{\mathalpha{\bm q}}
\nc{\bmr}{\mathalpha{\bm r}}
\nc{\bms}{\mathalpha{\bm s}}
\nc{\bmt}{\mathalpha{\bm t}}
\nc{\bmu}{\mathalpha{\bm u}}
\nc{\bmv}{\mathalpha{\bm v}}
\nc{\bmw}{\mathalpha{\bm w}}
\nc{\bmx}{\mathalpha{\bm x}}
\nc{\bmy}{\mathalpha{\bm y}}
\nc{\bmz}{\mathalpha{\bm z}}

\nc{\bmA}{\mathalpha{\bm A}}
\nc{\bmB}{\mathalpha{\bm B}}
\nc{\bmC}{\mathalpha{\bm C}}
\nc{\bmD}{\mathalpha{\bm D}}
\nc{\bmE}{\mathalpha{\bm E}}
\nc{\bmF}{\mathalpha{\bm F}}
\nc{\bmG}{\mathalpha{\bm G}}
\nc{\bmH}{\mathalpha{\bm H}}
\nc{\bmI}{\mathalpha{\bm I}}
\nc{\bmJ}{\mathalpha{\bm J}}
\nc{\bmK}{\mathalpha{\bm K}}
\nc{\bmL}{\mathalpha{\bm L}}
\nc{\bmM}{\mathalpha{\bm M}}
\nc{\bmN}{\mathalpha{\bm N}}
\nc{\bmO}{\mathalpha{\bm O}}
\nc{\bmP}{\mathalpha{\bm P}}
\nc{\bmQ}{\mathalpha{\bm Q}}
\nc{\bmR}{\mathalpha{\bm R}}
\nc{\bmS}{\mathalpha{\bm S}}
\nc{\bmT}{\mathalpha{\bm T}}
\nc{\bmU}{\mathalpha{\bm U}}
\nc{\bmV}{\mathalpha{\bm V}}
\nc{\bmW}{\mathalpha{\bm W}}
\nc{\bmX}{\mathalpha{\bm X}}
\nc{\bmY}{\mathalpha{\bm Y}}
\nc{\bmZ}{\mathalpha{\bm Z}}


\nc{\bmalpha}{{\mbox{\boldmath $\alpha$}}}
\nc{\bmbeta}{{\mbox{\boldmath $\beta$}}}
\nc{\bmgamma}{{\mbox{\boldmath $\gamma$}}}
\nc{\bmGamma}{{\mbox{\boldmath $\Gamma$}}}
\nc{\bmdelta}{{\mbox{\boldmath $\delta$}}}
\nc{\bmDelta}{{\mbox{\boldmath $\Delta$}}}
\nc{\bmeps}{{\mbox{\boldmath $\epsilon$}}}
\nc{\bmepsilon}{\bmeps}
\nc{\bmphi}{{\mbox{\boldmath $\phi$}}}
\nc{\bmPhi}{{\mbox{\boldmath $\Phi$}}}
\nc{\bmlambda}{{\mbox{\boldmath $\lambda$}}}
\nc{\bmLambda}{{\mbox{\boldmath $\Lambda$}}}
\nc{\bmmu}{{\mbox{\boldmath $\mu$}}}
\nc{\bmnu}{{\mbox{\boldmath $\nu$}}}
\nc{\bmpi}{{\mbox{\boldmath $\pi$}}}
\nc{\bmrho}{{\mbox{\boldmath $\rho$}}}
\nc{\bmpsi}{{\mbox{\boldmath $\psi$}}}
\nc{\bmPsi}{{\mbox{\boldmath $\Psi$}}}
\nc{\bmsigma}{{\mbox{\boldmath $\sigma$}}}
\nc{\bmSigma}{{\mbox{\boldmath $\Sigma$}}}
\nc{\bmtheta}{{\mbox{\boldmath $\theta$}}}
\nc{\bmTheta}{{\mbox{\boldmath $\Theta$}}}
\nc{\bmeta}{{\mbox{\boldmath $\eta$}}}
\nc{\bmxi}{{\mbox{\boldmath $\xi$}}}
\nc{\bmXi}{{\mbox{\boldmath $\Xi$}}}

\nc{\bmone}{{\bf 1}}
\nc{\bmhalf}{{\bf\frac{1}{2}}}
\nc{\bmnull}{{\bf 0}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% Cal stuff
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\nc{\calA}{\mathalpha{\cal{A}}}
\nc{\calB}{\mathalpha{\cal{B}}}
\nc{\calC}{\mathalpha{\cal{C}}}
\nc{\calD}{\mathalpha{\cal{D}}}
\nc{\calE}{\mathalpha{\cal{E}}}
\nc{\calF}{\mathalpha{\cal{F}}}
\nc{\calG}{\mathalpha{\cal{G}}}
\nc{\calH}{\mathalpha{\cal{H}}}
\nc{\calI}{\mathalpha{\cal{I}}}
\nc{\calJ}{\mathalpha{\cal{J}}}
\nc{\calK}{\mathalpha{\cal{K}}}
\nc{\calL}{\mathalpha{\cal{L}}}
\nc{\calM}{\mathalpha{\cal{M}}}
\nc{\calN}{\mathalpha{\cal{N}}}
\nc{\calO}{\mathalpha{\cal{O}}}
\nc{\calP}{\mathalpha{\cal{P}}}
\nc{\calQ}{\mathalpha{\cal{Q}}}
\nc{\calR}{\mathalpha{\cal{R}}}
\nc{\calS}{\mathalpha{\cal{S}}}
\nc{\calT}{\mathalpha{\cal{T}}}
\nc{\calU}{\mathalpha{\cal{U}}}
\nc{\calV}{\mathalpha{\cal{V}}}
\nc{\calW}{\mathalpha{\cal{W}}}
\nc{\calX}{\mathalpha{\cal{X}}}
\nc{\calZ}{\mathalpha{\cal{Z}}}
\nc{\calY}{\mathalpha{\cal{Y}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% Figure related stuff
%%%  -- Remember to set \figpath 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\nc{\epsfignocap}[2] {
\begin{nopagebreak}
  \begin{figure}[hbpt]
    \begin{center}
      \leavevmode \epsfxsize=#1 mm
      \epsffile{\figpath/#2.eps} 
    \end{center}
  \end{figure}
\end{nopagebreak}
}

\nc{\pstexfignocap}[2][1.0] {
\begin{nopagebreak}
  \begin{figure}[hbpt]
    \begin{center}
      \scalebox{#1}{
      \input{\figpath/#2.pstex_t}
} 
    \end{center}
  \end{figure}
\end{nopagebreak}
}

\nc{\pstexfig}[3][1.0]{
\begin{nopagebreak}
  \begin{figure}[hbpt]
    \begin{center}
    \ifthenelse{\boolean{DEBUG}}{
    \IfFileExists{\figpath/#2.pstex_t}{
    \scalebox{#1}{      
       \input{\figpath/#2.pstex_t}}}
       {
       \framebox[\linewidth][c]{\rule[-1cm]{0cm}{2cm}Figure missing: #2.pstex}}}
       {
       \scalebox{#1}{      
        \input{\figpath/#2.pstex_t}}
	}
	\caption{#3}
      \label{fig:#2}
    \end{center}
  \end{figure}
\end{nopagebreak}
}

\nc{\epsfigure}[3][1.0]{
\begin{nopagebreak}
  \begin{figure}[hbpt]
    \begin{center}
\leavevmode 
\scalebox{#1}{      
      \epsffile{\figpath/#2.eps}}
        \caption{#3}
      \label{fig:#2}
    \end{center}
  \end{figure}
\end{nopagebreak}
}


\nc{\epsfrag}[4][1.0]{
\begin{nopagebreak}
  \begin{figure}[htbp]
    \begin{center}
      \leavevmode 
      \ifthenelse{\boolean{DEBUG}}{
        \IfFileExists{\figpath/#4.eps}{
          #3
          \includegraphics[scale=#1]{\figpath/#4.eps}}
        {
          \framebox[\linewidth][c]{\rule[-1cm]{0cm}{2cm}Figure
            missing: #4.eps}}}
      {
        #3
        \includegraphics[scale=#1]{\figpath/#4.eps}}
      \caption{#2}
      \label{fig:#4}
    \end{center}
  \end{figure}
\end{nopagebreak}
}



% \nc{\epsfrag}[4][1.0]{
% \begin{nopagebreak}
%   \begin{figure}[htbp]
%     \begin{center}
%     \leavevmode 
%     #3
%     \includegraphics[scale=#1]{\figpath/#4.eps}
%         \caption{#2}
% 	  \label{fig:#4}
%     \end{center}
%   \end{figure}
% \end{nopagebreak}
% }


